Benders decomposition for Network Design Covering Problems

We consider two covering variants of the network design problem. We are given a set of origin/destination pairs, called O/D pairs, and each such O/D pair is covered if there exists a path in the network from the origin to the destination whose length is not larger than a given threshold. In the first problem, called the Maximal Covering Network Design problem, one must determine a network that maximizes the total fulfilled demand of the covered O/D pairs subject to a budget constraint on the design costs of the network. In the second problem, called the Partial Covering Network Design problem, the design cost is minimized while a lower bound is set on the total demand covered. After presenting formulations, we develop a Benders decomposition approach to solve the problems. Further, we consider several stabilization methods to determine Benders cuts as well as the addition of cut-set inequalities to the master problem. We also consider the impact of adding an initial solution to our methods. Computational experiments show the efficiency of these different aspects.

==> biblio.tex <==
\begin{thebibliography}{1}


\bibitem{Balas2002}%balas2002lift
E. Balas and  M. Perregaard. Lift-and-project for Mixed 0–1 programming: recent progress. \textit{Discrete Applied Mathematics}, 123(1-3), 129–154, 2002. 
% https://doi.org/10.1016/S0166-218X(01)00340-7

\bibitem{Balas2003}%balas2003precise
E. Balas and  M. Perregaard. A precise correspondence between lift-and-project cuts, simple disjunctive cuts, and mixed integer gomory cuts for 0-1 programming. \textit{Mathematical Programming}, 94(2-3), 221–245, 2003. 
% https://doi.org/10.1007/s10107-002-0317-y

\bibitem{Barahona1996network}
 F. Barahona. Network Design Using Cut Inequalities. \textit{SIAM Journal on Optimization}, 6(3), 823–837, 1996.
% https://doi.org/10.1137/S1052623494279134

\bibitem{Ben2007acceleration}
W. Ben‐Ameur, J. Neto, L. Gouveia, and S. Voss. Acceleration of cutting‐plane and column generation algorithms: Applications to network design. \textit{Networks}, 49(1), 3–17, 2007.
% https://doi.org/10.1002/net.20137

\bibitem{Ben1962}%Ben
J. F. Benders. Partitioning procedures for solving mixed-variables programming problems. \textit{Numerische Mathematik}, {\bf
4}, 232--252, 1962.

\bibitem{Berge1957}
C. Berge. Two theorems in Graph Theory.  \textit{Proceedings of the National Academy of Sciences of the United States of America}, {\bf 43(9)} 842--844, 1957.

\bibitem{Berman2009}%BDKW
O. Berman , Z. Drezner, D. Krass and G.O. Wesolowski. The variable radius covering problem. \textit{European Journal of Operational Research}, {\bf 196}, 516--525, 2009.

\bibitem{Canca2017}%CDLM17
D. Canca, A. De-los-Santos, G. Laporte and J. A. Mesa. An adaptive neighborhood search metaheuristic for the integrated
rapid transit network design and line planning problem, \textit{Computers \& Operations Research}, {\bf 78}, 1--14, 2017.


\bibitem{Canca2019}%CDLM19
D. Canca, A. De-los-Santos, G. Laporte and J. A. Mesa. Integrated railway rapid transit network design and line planning problem with maximum profit, \textit{Transportation Research Part E: Logistics and Transportation Review}, {\bf 127}, 1--30, 2019.

\bibitem{Cascetta2009}%Cas
E. Cascetta. \textit{Transportation System Analysis: Models and Applications}, Springer, 2009.

\bibitem{Church2018}%ChMu
 R. Church and A. Murray. \textit{Location Covering Models}, Springer, 2018.
 
\bibitem{Church1974}%ChRe
R. Church and C. ReVelle. The maximal covering location problem. \textit{Papers of the Regional Science Association}. {\bf 32}, 101--118, 1974.

\bibitem{Conforti2019facet}
M. Conforti and L. Wolsey. “Facet” separation with one linear program. \textit{Mathematical Programming}, 178(1), 361–380, 2019.
% https://doi.org/10.1007/s10107-018-1299-8

\bibitem{Cordeau2019benders}
J. F. Cordeau, F. Furini and I. Ljubić. Benders decomposition for very large scale partial set covering and maximal covering location problems. \textit{European Journal of Operational Research}, 275(3), 882-896, 2019.

\bibitem{Costa2009benders}
A. Costa, J. Cordeau and B. Gendron. Benders, metric and cutset inequalities for multicommodity capacitated network design. \textit{Computational Optimization and Applications}, 42(3), 371–392, 2009.

\bibitem{Desrochers1988algorithm}
Martin Desrochers. \textit{An algorithm for the shortest path problem with resource constraints}, {\'E}cole des hautes {\'e}tudes commerciales, Groupe d'{\'e}tudes et de recherche en analyse des décisions, 1988.


\bibitem{Farahani2012}%FAHHG
R. Z. Farahani, N. Asgari, N. Heidari, M. Hosseininia and M. Goh. Covering problems in facility location: a review. \textit{Computers and Industrial Engineering}, {\bf 62} 368--407, 2012.

\bibitem{Fischetti2010note}
M. Fischetti, D. Salvagnin and A. Zanette. A note on the selection of Benders’ cuts. \textit{Mathematical Programming}, 124(1-2), 175–182, 2010.

\bibitem{Garcia2013}%GaLMP
B. García-Archilla, A. J. Lozano, J. A. Mesa and F. Perea. GRASP algorithms for the robust railway network design problem. \textit{Journal of Heuristics}, {\bf 19}, 399--422, 2013.

%\JAM{
% \bibitem{GarciaMarin2020} 
% S. García, A. Marín. Covering Location Problems,

\bibitem{Hakimi1965}%Hak
S. L. Hakimi. Optimum distribution of switching centers in a communication network and some related graph theoretic problems.
\textit{Operations  Research}, {\bf 13}, 462--475, 1965.

\bibitem{Hakimi1993}
S. L. Hakimi, E. F. Schmeichel and M. Labbé. On locating path‐or tree‐shaped facilities on networks. \textit{Networks}, 23(6), 543-555, 1993.

\bibitem{Johnson1978}%JLR
D. S. Johnson, J. K. Lenstra and A. H. G. Rinooy Kan. The complexity of the network design problem, \textit{Networks}, {\bf 8}, 279--285, 1978.

\bibitem{Karp1971}%Karp
R. M. Karp. Reducibility among combinatorial problems. \textit{Complexity of Computers Computations} (R. E. Miller, J. W. Tatcher, J. D. Bohlinger, eds.), 85--103, Plenum, New York, 1971.

\bibitem{Koster2013extended}
A. Koster, T. Phan and M. Tieves. Extended Cutset Inequalities for the Network Power Consumption Problem. \textit{Electronic Notes in Discrete Mathematics}, 41(C), 69–76, 2013.

\bibitem{Krol2019}%KK
 A. Król and M. Król. The design of a metro network using a genetic algorithm. \textit{Applied Science}, 9, 433, 2019.

\bibitem{Ljubic2012exact}
I. Ljubić, P. Putz and J. Salazar‐González. Exact approaches to the single‐source network loading problem. \textit{Networks}, 59(1), 89–106, 2012.

\bibitem{Magnanti1986}%MagMirWong 
T. L. Magnanti, P. Mireault and R. T. Wong. Tailoring Benders decomposition for uncapacitated network design. \textit{Netflow at Pisa}. Mathematical Programming Studies (G. Gallo, C. Sandi, eds.), vol 26, Springer, Berlin, Heidelberg, 1986.

\bibitem{Magnanti1981accelerating}
T. L. Magnanti and R. T. Wong. Accelerating Benders Decomposition: Algorithmic Enhancement and Model Selection Criteria. \textit{Operations Research}, 29(3), 464–484, 1981.

\bibitem{Magnanti1984}%MagWong
T. L. Magnanti and R. T. Wong. Network Design and Transportation Planning: Models and Algorithms. \textit{Transportation Science}, {\bf 18}, 1--55, 1984.


\bibitem{Marin2009}%MJ
A. Marín and P. Jaramillo. Urban rapid transit network design: acceleraded Benders decomposition. \textit{Annals of Operations Research}, {\bf
169} 35--53, 2009.

\bibitem{Melkote2001}%MelDas
S. Melkote and M. S. Daskin. An integrated model of facility location and transportation network design. \textit{Transportation Research, Part A}, {\bf 35}, 515--538, 2001.

\bibitem{Mesa2018}
J. A. Mesa. Comments: on Extensive facility location on networks: an updated review 1. \textit{TOP}, {\bf 6(2)}, 227--228, 2018.

\bibitem{Mesa1991}%MeBo
J. A. Mesa and B. T. Boffey.  A review of extensive facility location in networks. \textit{European Journal of Operational Research} {\bf 95}, 592--603, 1991.

\bibitem{Norman1959}%NorRa
R. Z. Norman and M. O. Rabin. An algorithm for a minimum cover of a graph. \textit{Proceedings of the American Mathematical Society}, {\bf 10}, 315--319, 1959.

\bibitem{Perea2020}%PMMR
F. Perea, M. Menezes, J. A. Mesa and F. Rubio-del-Río. Transportation infrastructure network design in presence of modal competition: computational complexity classification and a genetic algorithm. \textit{TOP}, {\bf 28}, 442--474, 2020.

\bibitem{Puerto2018}%PRS
J. Puerto, F. Ricca and A. Scozzari. Extensive facility location on networks: and updated review. \textit{TOP}, {\bf 6(2)}, 187-226, 2018.

\bibitem{Rahmaniani2017}%RCGR
R. Rahmaniani, T. G. Crainic, M. Gendreau and W. Rei. The Benders decomposition algorithm: A literature review. \textit{European Journal of
Operational Research}, {\bf 259} 801--817, 2017.


\bibitem{Schilling1993}%SchJaBar
D. A. Schilling, V. Jayamaran and R. Barkhi. A review of covering problems in facility location. \textit{Location Science}. {\bf 1}, 25--55, 1993.

\bibitem{sioux}
Sioux Networks, \url{http://www.bgu.ac.il/~bargera/tntp/SiouxFalls_CNDP/SiouxFallsVariantsForNetworkDesign.html}


\bibitem{Toregas1971}%TSRB
C. Toregas, R. Swain, C. ReVelle and L. Bergman. The location of emergency services facilities.
\textit{Operations Research}, {\bf 19}, 1363--1373, 1971.

\bibitem{FORTZ2009359}%TSRB
B. Fortz and M. Poss. An improved Benders decomposition applied to a multi-layer network design problem
\textit{Operations Research Letters}, {\bf 37}, 359 -- 364, 2009.

\bibitem{botton2013benders}%TSRB
Botton, Quentin and Fortz, Bernard and Gouveia, Luis and Poss, Michael. Benders decomposition for the hop-constrained survivable network design problem.
\textit{INFORMS journal on computing}, {\bf 25}, 13--26, 2013.

\bibitem{schmidt2014location}%TSRB
Schmidt, Marie and Sch{\"o}bel, Anita. Location of speed-up subnetworks.
\textit{Annals of Operations Research}, {\bf 1}, 379--401, 2014.


\end{thebibliography}

==> literature.tex <==

%Covering problems in graphs have attracted the attention of
%researchers since the middle of last century. As far as the
%authors are aware the first papers on the vertex-covering problem
%were due to Berge \cite{Berge1957} and Norman and Rabin \cite{Norman1959} in the latest 50s. This problem is related with the set-covering problem in which a family of sets is given and the minimal subfamily \ML{whose} union contains all the elements is sough \ML{for}.
% The decision versions of both problems were  proved to be NP-complete \cite{Karp1971}. In \cite{Hakimi1965} the vertex-covering problem was formulated as an integer linear programming model and solved by
%using Boolean functions.

%Authors in \cite{Toregas1971} applied the vertex-covering problem to the location of emergency services. They assumed that a vertex is covered if it is within a given coverage distance. Church and ReVelle introduced the maximal covering location problem by fixing the number of facilities to be located \cite{Church1974}. Each vertex has an associated population and the objective is to cover the maximum population within a fixed distance threshold. Since then many variants and extensions of the vertex-covering and maximal covering  problems have been
%researched (see \cite{Schilling1993}, \cite{Berman2009}, \cite{Farahani2012}, \cite{Church2018}, and the references therein).

%An  extensive facility location problem consists of locating a subgraph such as to optimize some objective function with some contraints regarding demand points \cite{Mesa1991}, \cite{Puerto2018}. Problems where a path or a tree-graph with a possibly  limited length so that the maximum distance or the sum of distances to the vertices is minimized generalize, to non-point
%facilities, the concept of center and median,  respectively. In these papers extensive location problems with other
%objective functions as k-centrum, ordered median and equity
%measures have also been reviewed. Several papers have dealt with
%extensive facility location with covering objectives (see \cite{Mesa2018}, and the references therein). The extensive vertex-covering and maximal covering problems are extensions of the point vertex-covering and maximal covering problems where the number
%of vertices of the coverage is substituted by the length or other characteristic of the covering subgraph.
%These problems depend on the type of underlying graph, the location of the demand, the shape of the graph used for covering and its tips (discrete or continuous), the way of covering and other characteristics. Indirect and direct covering of a graph by a subtree with limited number of vertices or bounded length problems are NP-hard in general, since they are special cases of the Steiner tree problem. However, if the underlying graph is a tree some of the problems can be solved by polynomial time algorithms, those cases in which paths are being sought \cite{Hakimi1993}. If the search consists of a tree there are some NP-hard problems, among which stands out Median Problem.

%Network design is a broad and spread subject whose models often depend on the field in which they are applied. However, a systematization was done by authors in \cite{Magnanti1984} where some classical graph problems as the minimal spanning tree, Steiner tree, shortest path and traveling salesman problems
 %are included as particular cases of a general mathematical programming model.
 %Discrete network design problems assume that a given underlying graph is given,
 %and could  be classified into four groups with increasing complexity: without capacity, with capacity, capacity or coverage expansion, and multiperiod. Extensive facility location and network design are interlaced subjects where synergies often appear. Moreover, network design and point-location problems are
 %very related since the transportation network is the way to access the facilities and, therefore the efficiency of the optimal point depends on the network design. In fact several models integrate the location of facilities and the design of the network used to fulfill the demand. The objective function of the model in \cite{Melkote2001} includes transportation cost, facility location, and construction of the network. However, very early was stated the NP-hardness of a special network design problem. Authors in \cite{Johnson1978} showed that the knapsack problem is reducible to the problem of choosing a subgraph that minimizes the sum of the shortest path weights between all vertex pairs subject to a budget constraint.

%All the previously reviewed research considers a
%customer-to-server system, where demand uses the network to access
%the point or extensive facilities. However, in many cases reaching
% or been closed to a facility is not enough to complete the
%service. In many telecommunication, transportation, public
%services  and other systems the demand uses the facility as an
%intermediate instead of a final step. 

%For example, this is the case of public urban transportation network where a customer have to spend time to reach the stop/station from its origin, then
%wait for the next service, spend  in-vehicle time, and finally
%reach its destination. Network design of these systems are even
%more complex than those where the customers have just to go to the
%servers.

%In these cases the demand is given by pairs instead of
%points, and usually each pair has an associated weight indicating
%the traffic between the origin and the destination. Usually this
%demand is encoded using an origin-destination matrix. When planning a new network, often there exists a network already functioning and
%offering its service to the same set of origin-destination pairs.
%For example, in order to improve the mobility of a big city or
%metropolitan area, a new rapid transit systems is planned. The
%current transit system could be more dense than the rapid transit
%planned but slower since uses the same right-of-way than the
%private traffic. Thus, in some way both systems compete between
%them and both compete with the private mode of transportation.
%A similar effect occurs with mobile telecommunication operators. 
%Therefore, the traffic between an origin and a destination is distributed among the several systems that provide the service. 

%There are mainly two ways of allocating the share of each mode. The first one is the binary all-or-nothing way, where the demand is served by each mode only if the mode the demand point within a range of quality service, as in \cite{church1974maximal}. The second one is some continuous function, for example multi-logit probability distributions, as in \cite{cascetta2009transportation}. Both mode-share are based in the comparison of distances, times, costs, generalized costs or utilities. In this paper,  we consider a binary one, where each pair is served only if the time spent into the network is below a threshold. This threshold represents the comparison between the time spent in the proposed network and a private mode assigning the full share to the most beneficial one. When the aim is to maximize the sum of the
 %weights of the covered pairs by the new network, and the constraint is the total cost of the network the problems of finding an optimal network without cycles and allowing cycles are NP-Hard \cite{perea2020transportation}. 
 
 Since most network design problems are NP-hard,  recent research efforts have been oriented to apply metaheuristic algorithms to obtain good solutions in a reasonable computational time. Thus, in the field of transportation network design, Genetic Algorithms (\cite{krol2019design}), Greedy Randomized Adaptive Search Procedures
 (\cite{garcia2013grasp}),  Adaptive Large Neighborhood Searchs  (\cite{canca2017adaptive}) and
  metaheuristics (\cite{canca2019integrated}) have been applied to rapid transit network design problems with applications to medium-size instances.  
  
  In this article we propose exact methods based on Benders' decomposition. Benders proposed this decomposition for solving mixed-integer mathematical programming problems in the early 60s \cite{benders2005partitioning}. Since then, it has been applied to many problems in different fields, see \cite{rahmaniani2017benders}  for a recent literature review on the use of Benders decomposition in combinatorial optimization. One remarkable recent contribution applied to set covering and maximal covering location problems  appears in \cite{Cordeau2019benders}.

 Benders decomposition for network design problems have been studied since the 80s. In \cite{magnanti1986tailoring}, authors minimize the total building cost of an uncapacitated network subject to the constraints that all O/Ds pairs must be served. Given the structure of the problem, the Benders reformulation is stated with one sub-problem for each pair O/D. A Benders decomposition for a multi-layer network design problem is 
presented in \cite{FORTZ2009359}. Benders decomposition were also applied in \cite{botton2013benders} in the context of designing survivable networks. Authors in \cite{Costa2009benders} have studied multi-commodity capacitated network design and the strength of different Benders cuts; in \cite{marin2009urban} a multi-objective approach is solved through Benders decomposition where coverage is maximized, but at the same time total cost design is minimized. To best of our knowledge, this is the first time that a branch-and-Benders-cut approach is applied to network design coverage problems. We also study for the first time in this context the inclusion of {\it facet-defining cuts} as was recently proposed by \cite{Conforti2019facet}.


==> literature_JA.tex <==

Covering problems in graphs have attracted the attention of
researchers since the middle of last century. As far as the
authors are aware the first papers on the vertex-covering problem
were due to Berge (1957)  \cite{Berge} and Norman and Rabin (1959) \cite{NorRa}  The problem
dealt with in these papers was to find a subset of vertices with
minimum cardinality such that each edge is incident to at least
one vertex of it. This problem is related with the set-covering problem in which a family of sets is given and the minimal subfamily which union contains all the elements is sough.
Current file
Overview
2

 The decision versions of both problems were  proved to be   NP-complete (Karp (1972) \cite{Karp}). The
 vertex-covering problem was formulated as an integer linear programming model and solved by
using Boolean functions by Hakimi (1965)  \cite{Hak}.
This problem was applied to the location of emergency services by
Toregas et al. (1971) \cite{TSRB}. They assumed a vertex is
covered by other if they are within a given coverage distance. When the number of facilities
to be located is fixed then the maximal covering location problem
arises (Church and ReVelle, (1974) \cite{ChRe})  in which problem each vertex has an
 associated population and the objective is to cover the maximum
population within a fixed distance threshold. Since then many
variants and extensions of the vertex-covering and maximal covering  problems have been
researched (see, Schilling et al., (1993) \cite{SchJaBar}, Berman et al., (2009) \cite{BDKW},
Farahani et al. (2012) \cite{FAHHG}, and  Church and Murray, (2018) \cite{ChMu}, and the references therein).

An  extensive
facility location problem consists of locating a subgraph such
that optimizes some objective function with some contraints regarding demand points
(see, Mesa and Boffey, 1991 \cite{MeBo}, and Puerto et al.  (2018) \cite{PRS}.) Problems where a
path or a tree-graph with a possibly  limited length so that the maximum
distance or the sum of distances to the vertices is minimized
generalize,  to non-point
facilities, the concept of center and median,  respectively. In these papers extensive location problems with other
objective functions as k-centrum, ordered median and equity
measures have also been reviewed. Several papers have dealt with
extensive facility location with covering objectives (see, Mesa,
(2018) \cite{Mesa}, and the references therein). The extensive vertex-covering and maximal covering problems are extensions of the point vertex-covering and maximal covering problems where the number
of vertices of the coverage is substituted by the length or other characteristic of the covering subgraph.
The problems depend on the type of underlying graph, the location of the demand, the shape of the graph used for covering and its tips (discrete or continuous), the way of covering and other parameters.
Indirect and direct covering of a graph by a subtree with
limited number of vertices or bounded length problems are
 NP-hard in general, since they are special cases of the Steiner tree problem.
 However, if the underlying graph is a tree most of the problems can be solved by  polynomial time algorithms.

Network design is a broad and spread subject whose models often depend on the field in which they are applied. However,
a systematization was done by Magnanti and Wong (1984) \cite{MagWong}
where some classical graph problems as the minimal spanning tree, Steiner tree, shortest path and traveling salesman problems
 are included as a particular cases of a general mathematical programming model.
 Discrete network design problems assume that a given underlying graph is given,
 and could  be classified into four groups with increasing complexity: without capacity, with capacity,
 capacity or coverage expansion, and multiperiod. Extensive facility location and network design are
 interlaced subjects where synergies often appear. Moreover, network design and point-location problems are
 very related since the transportation network is the way to access the facilities and, therefore the efficiency of the optimal point depends on the network design. In fact several relatively recent models integrate the location of facilities and the design of the network used to fulfill the demand. The objective function of the model in the paper by Melkote and Daskin (2001) \cite{MelDas} includes transportation cost, facility location, and construction of the
 network. However, very early was stated the NP-hardness of a
 special network design problem. In the paper by Johnson et al. (1978) \cite{JLR}, it was shown that the knapsack problem is reducible to the problem of choosing a subgraph such that it minimizes the sum  of the shortest path weights between all vertex pairs subject to a budget constraint.

All the previously reviewed research considers a
customer-to-server system, where demand uses the network to access
the point or extensive facilities. However, in many cases reaching
or been closed to a facility is not enough to complete the
service. In many telecommunication, transportation, public
services  and other systems the demand uses the facility as an
intermediate instead of a final step. This is, for example, the
case of public urban transportation network, where a customer have
to spend  a time to reach the stop/station from its origin, then
wait for the next service, spend an in-vehicle time, and finally
reach its destination. Network design of these systems are even
more complex than those where the customers just have to go to the
servers. 

In this cases the demand is given by pairs instead of
points, and usually each pair has an associated weight indicating
the traffic between the origin and the destination. Usually this
demand is codify by an origin-destination matrix. When planning a
new network, often there exists a network already functioning and
offering its service to the same set of origin-destination pairs.
For example, in order to improve the mobility of a big city or
metropolitan area, a new rapid transit systems is planned. The
current transit system could be more dense than the rapid transit
planned but slower since uses the same right-of-way than the
private traffic. Thus, in some way both systems compete between
them and both compete with the private mode of transportation.
 Almost the same happens with mobile telecommunication operators. Therefore, the traffic between an origin and
 a destination is distributed among the several systems that provide the service. There are mainly two ways of
 allocating the share of each mode. The first one is the binary  all-or-nothing, the second one is some continuous
 function (see Cascetta, 2009, \cite{Cas}). Both mode-share are based in the comparison of distances, times, costs,
 generalized costs or utilities. The second is more for real but, in this paper,  we will use the binary one.
 Since the main aim of this paper is not to have a good representation of the reality but to assess the Benders'
 decomposition in a basic planning infrastructure network design, we will use the binary distribution.
 For this purpose, usually the utility of both modes are compared for each  o-d pair and  is assigned the
 share one to the most beneficial  and zero to another.  When the aim is to maximize the sum of the
  weights of the covered pairs by the new network, and the constraint is the total cost of the network the problems of finding
  an optimal network without cycles and allowing cycles are NP-Hard (Perea et al. (2020),
  \cite{PMMR}).Since most of the network design problems are
  NP-hard, the recent research efforts have been oriented to apply
  metaheuristic algorithms to obtain good solutions in a
  reasonable computational time. Thus, in the field of
  transportation network design, Genetic Algorithms (Król amd
  Król, (2019), \cite{KK}), Greedy Randomized Adaptive Search Procedure
  (Garc\'\i a-Archilla et al., 2013, \cite{GaLMP}),  Adaptive Large
  Neighborhood Search (Canca et al. 2017, \cite{CDLM17}) and
  matheuristic (Canca et al. 2019, \cite{CDLM19}) have been applied
  to rapid transit network design problems with applications to
  medium-size instances. Although exact methods cannot solve
  nowadays large instances in a short time, infrastructure network
  design problems belong to the strategic phase of the sequential
  process of transportation planning and, therefore, computational
  time is less important than to other problems belonging to
  operational or on-line phases. Moreover, exact methods require a
  more profound knowledge, and thus provide more insight on the
  problems and mathematical models. Benders decomposition was
  proposed by Benders (1962, \cite{Ben}) for solving mixed-integer
  mathematical programming problems. Since then, it has been
  applied to many problems in different fields, see \cite{RCGR}
  for a recent literature review on the use of Benders
  decomposition in combinatorial optimization. One remarkable recent contribution appears in \cite{cordeau2019benders} in the context of set covering and maximal covering. 

 Benders decomposition for network design problems have been studied since the 80s. In \cite{MagMirWong}, authors minimize the total building cost of an uncapacitated network subject to the constraints that all O/Ds pairs must be served. Given the structure of the problem, the Benders reformulation is stated with one sub-problem for each pair O/D. Authors in \cite{costa2009benders} studied multicommodity capacitated network design and study the strength of different Benders cuts; in \cite{MJ} a multi-objective approach is solved through Benders decomposition where coverage is maximized, but at the same time total cost design is minimized. To best of our knowledge, this is the first time that a branch-and-Benders-cut approach is applied to network design coverage problems. We also study for the first time in this context the inclusion of {\it facet-define cuts} as it was recently proposed by \cite{conforti2019facet}.

==> old_tables.tex <==
\begin{table}[htpb]
\centering
\begin{tabular}{cccccc}
\cline{2-6}
 & \texttt{CPLEX}& \texttt{Auto\_BD} & \texttt{BD\_Trd} & \texttt{BD\_Norm} & \texttt{BD\_CW}\\ \hline
 without \texttt{CS} &3& 10 & 9 & 8 & 8 \\ 
\texttt{+CS}& - & 10 & 10 & 10 & 10 \\ \hline
\end{tabular}\caption{Instances N40 solved for $(MC)$ within a time limit of 1 hour.}
\label{table:optMC}
\end{table}

\begin{table}[htpb]
\centering
\begin{tabular}{cccccc}
\cline{2-6}
 & \texttt{CPLEX}& \texttt{Auto\_BD} & \texttt{BD\_Trd} & \texttt{BD\_Norm} & \texttt{BD\_CW}\\ \hline
 without \texttt{CS}&3& 9 & 8 & 8 & 8 \\ %\hline
\texttt{+CS} & - & 10 & 10 & 10 & 10 \\ \hline
\end{tabular}\caption{Instances N40 solved for $(PC)$ within a time limit of 1 hour.}
\label{table:optPC}
\end{table}

\begin{table}[htpb]
\centering
\begin{tabular}{c c c cc cc cc cc}
\cline{2-11}% \hline
&\multirow{2}{*}{Network} & \texttt{CPLEX} & \multicolumn{2}{c}{\texttt{Auto\_BD}} & \multicolumn{2}{c}{\texttt{BD\_Trd}} & \multicolumn{2}{c}{\texttt{BD\_Norm}} & \multicolumn{2}{c}{\texttt{BD\_CW}} \\ \cline{3-11} 
 & & \texttt{t} & \texttt{t} & \texttt{cuts} & \texttt{t} & \texttt{cuts} & \texttt{t} & \texttt{cuts} & \texttt{t} & \texttt{cuts} \\ \hline
\multirow{3}{1cm}{\centering{without \texttt{CS}}} & N10 & 0.18 & 0.43 & 27 & 0.25 & 92 & 0.24 & 91 & 0.19 & 94 \\ 
& N20 & 6.77 & 4.51 & 273 & 3.89 & 620 & 3.18 & 590 & 3.34 & 641 \\ 
& N40 & 1646.93 & 617.85 & 1967 & 1095.25 & 3990 & 541.03 & 3677 & 457.81 & 4137 \\ \hline
\multirow{3}{*}{\texttt{+CS}}& N10 & - & 0.32 & 12 & 0.21 & 49 & 0.28 & 52 & 0.23 & 54 \\ 
& N20 & - & 3.94 & 178 & 2.29 & 382 & 2.50 & 383 & 1.85 & 416 \\
& N40 & - & 484.95 & 1248 & 637.49 & 2378 & 575.87 & 2530 & 272.39 & 3186 \\ \hline
\end{tabular}\caption{Comparing the performance of the three algorithms for $(MC)$.}
\label{table: MC 1}
\end{table}

\begin{table}[htpb]
\centering
\begin{tabular}{c c c cc cc cc cc}
\cline{2-11}
& \multirow{2}{*}{Network} & \texttt{CPLEX} & \multicolumn{2}{c}{\texttt{Auto\_BD}} & \multicolumn{2}{c}{\texttt{BD\_Trd}} & \multicolumn{2}{c}{\texttt{BD\_Norm}} & \multicolumn{2}{c}{\texttt{BD\_CW}} \\ \cline{3-11} 
 & & \texttt{t}& \texttt{t} & \texttt{cuts} & \texttt{t} & \texttt{cuts} & \texttt{t} & \texttt{cuts} & \texttt{t} & \texttt{cuts} \\ \hline
 \multirow{3}{1.3cm}{\centering{without \texttt{CS}}} & N10 & 0.18 & 0.29 & 16 & 0.24 & 92 & 0.28 & 89 & 0.20 & 91 \\ %\hline
 & N20 & 6.73 & 4.87 & 305 & 3.55 & 607 & 4.68 & 681 & 2.15 & 606 \\ %\hline
& N40 & 2153.15 & 504.06 & 1752 & 657.59 & 4470 & 514.42 & 4246 & 837.41 & 4412 \\ \hline
\multirow{3}{*}{\texttt{+CS}}& N10 & - & 0.28 & 11 & 0.16 & 56 & 0.20 & 57 & 0.145 & 54 \\
& N20& - & 4.12 & 213 & 3.11 & 497 & 3.43 & 495 & 2.070 & 461 \\
& N40 & - & 439.23 & 1527 & 261.74 & 3528 & 323.21 & 3583 & 197.55 & 3949 \\ \hline
\end{tabular}
\caption{Comparing the performance of the three algorithms for $(PC)$.}
\label{table: PC 1}
\end{table}














\begin{table}[htpb]
\centering
\begin{tabular}{c cc cc cc cc}
\cline{2-9}
& \multicolumn{2}{c}{\texttt{Auto\_BD}} & \multicolumn{2}{c}{\texttt{BD\_Trd}} & \multicolumn{2}{c}{\texttt{BD\_Norm}} & \multicolumn{2}{c}{\texttt{BD\_CW}} \\ \cline{2-9} 
& \texttt{gap} & \texttt{cuts} & \texttt{gap} & \texttt{cuts} & \texttt{gap} & \texttt{cuts} & \texttt{gap} & \texttt{cuts} \\ \hline
without\{\texttt{CS}, \texttt{IS}, \texttt{RNC}\}& 38.54 & 6545 & 45.68 & 14068 & 44.53 & 13340 & 43.77 & 16707 \\ 
\texttt{+CS}& 30.06 & 3729 & 24.27 & 8754 & 22.17 & 8912 & 25.76 & 11378 \\ 
\texttt{+CS+IS} & 32.90 & 4987 & 27.23 & 9038 & 26.94 & 9469 & 22.27 & 11151 \\
\texttt{+CS+IS+RNC} &\multicolumn{2}{c}{-}& 37.88 & 8054 & 37.92 & 8230 & 33.58 & 10834 \\ \hline
\end{tabular}\caption{Computing gaps to solve N60 $(MC)$ instances comparing the performance of three families of Benders cuts.}
\label{table:MC 2}
\end{table}



\begin{table}[htpb]
\centering
\begin{tabular}{c cc cc cc cc}
\cline{2-9}
& \multicolumn{2}{c}{\texttt{Auto\_BD}} & \multicolumn{2}{c}{\texttt{BD\_Trd}} & \multicolumn{2}{c}{\texttt{BD\_Norm}} & \multicolumn{2}{c}{\texttt{BD\_CW}} \\ \cline{2-9} 
& \texttt{gap} & \texttt{cuts} & \texttt{gap} & \texttt{cuts} & \texttt{gap} & \texttt{cuts} & \texttt{gap} & \texttt{cuts} \\ \hline
without\{\texttt{CS}, \texttt{IS}, \texttt{RNC}\} & 20.49 & 7009 & 20.40 & 14784 & 21.41 & 15501 & 19.93 & 15116 \\ %\cline{1-3}
\texttt{+CS} & 15.92 & 5109 & 14.89 & 12354 & 14.09 & 11687 & 14.50 & 11744 \\ %\cline{2-3}
\texttt{+CS+IS} & 15.86 & 4372& 11.06 & 8961 & 10.47 & 8490 & 10.44 & 9683 \\ %\cline{3-3}
\texttt{+CS+IS+RNC} &\multicolumn{2}{c}{-} & 20.93 & 10971 & 21.28 & 11449 & 19.94 & 11053 \\ \hline
\end{tabular}\caption{Computing gaps to solve N60 $(PC)$ instances comparing the performance of three families of Benders cuts.}
\label{table:PC 2}
\end{table}

==> paper Benders Decomposition draft ArXiv - tercera versi�n/benders.tex <==
\section{Benders Implementations}\label{sec:BImp}
In the following, we describe different Benders implementations for $(MC)$ and $(PC)$ obtained by projecting out variables $f^w_a$. Given that $(MC)$ and $(PC)$ share the same subproblem structure the Benders decomposition applied to $(MC)$ is valid for $(PC)$ and vice versa. Thus, we will apply the same Benders decomposition for both problems throughout this manuscript. These implementations are used as sub-routines in a branch-and-Benders-cut scheme. This scheme allows cutting infeasible solutions along the branch-and-bound tree. Depending on the implementation, infeasible solutions can be separated at any node in the branch-and-bound tree or only when an integer solution is found. In the case of $(MC)$, the master problem that we solve is:
\begin{align}
(M\_MC) \quad \max\limits_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}} & \quad \sum_{w\in W} g^w z^w \\
\mbox{s.t. } & \quad \mbox{(\ref{eq:budget}), \, (\ref{rel_xy}), \, (\ref{eq:nat})} & \nonumber\\
&\quad +\{\mbox{Benders Cuts }(\boldsymbol{x},\boldsymbol{y},\boldsymbol{z})\}. \nonumber
\end{align}
\noindent The master problem for $(PC)$, named $(M\_PC)$, is stated analogously.

In Section \ref{s:lpfeas}, we discuss the standard \textit{Benders cuts} obtained by dualizing the respective feasibility subproblem. Then, in Section \ref{s:normalben} we discuss ways of generating normalized subproblems, to produce stronger cuts. We name these cuts \textit{normalized Benders cuts}. In Section \ref{s:facertdef}, we apply {\it facet-defining cuts} in order to get stronger cuts, as it is proposed in \cite{Conforti2019facet}. Finally, we discuss an implementation where, at the beginning, \textit{cut-set inequalities} are added to enhance the link between $\boldsymbol{z}$ and $\boldsymbol{x}$, and then {\it Benders cuts} are added.

\subsection{LP feasibility cuts} \label{s:lpfeas}

Since the structure of the model allows it, we consider a feasibility subproblem made of constraints (\ref{flow_cons}), (\ref{Capacity}), (\ref{Utility}) and (\ref{eq:nneg-f}) for each commodity $w\in W$, denoted by $(SP)^w$. We note that each subproblem is feasible whenever $z^w=0$, so it is necessary $(SP)^w$ to check feasibility only in the case where $z^w>0$. As it is clear from the context, we remove the index $w$ from the notation. The dual of each feasibility subproblem can be expressed as: 
\begin{align}
(DSP)^w\quad \max\limits_{\boldsymbol{\alpha},\boldsymbol{\sigma},\boldsymbol{\upsilon}}&\quad z\,\alpha_{w^s} - \sum_{e \in E} x_e\,\sigma_e - u\, z\,\upsilon\\
\mbox{s.t. }&\quad \alpha_i - \alpha_j - \sigma_e - d_a\, \upsilon \le 0,& a=(i,j) \in A : e=\{i,j\}, \\
&\quad \sigma_e, \, \upsilon \ge 0, & e\in E,
\label{sub:trd}
\end{align}
\noindent where $\boldsymbol{\alpha}$ is the vector of dual variables related to constraints (\ref{flow_cons}), $\boldsymbol{\sigma}$ is the vector of dual variables corresponding to the set of constraints (\ref{Capacity}) and $\boldsymbol{\upsilon}$ is the dual variable of constraint (\ref{Utility}). Since constraints in (\ref{flow_cons}) are linearly dependent, we set $\alpha_{w^t}=0$. Given a solution of the master problem $(\boldsymbol{x},\boldsymbol{y},\boldsymbol{z})$, there are two possible outcomes for $(SP)^w$:
\begin{enumerate}
\item $(SP)^w$ is infeasible and $(DSP)^w$ is unbounded. Then, there exists an increasing direction $(\boldsymbol{\alpha},\boldsymbol{\sigma},\boldsymbol{\upsilon})$ with positive cost. In this case,
the current solution $(\boldsymbol{x},\boldsymbol{y},\boldsymbol{z})$ is cut by:
\begin{equation}
 (\alpha_{w^s} - u\,\upsilon)\,z - \sum_{e \in E} \sigma_e\, x_e \le 0. \label{eq:feasibility_cut}
\end{equation}
\item $(SP)^w$ is feasible and consequently, $(DSP)^w$ has an optimal objective value equal to zero. In this case, no cut is added. 
\end{enumerate}

\subsection{Normalized Benders cuts} \label{s:normalben}

The overall branch-and-Benders-cut performance heavily relies on how the cuts are implemented. It is known that feasibility cuts may have poor performance due to the lack of ability of selecting a {\it good} extreme ray (see for example \cite{Fischetti2010note, Ljubic2012exact}). However, normalization techniques are known to be efficient to overcome this drawback \cite{Magnanti1981accelerating, balas2002lift,balas2003precise}. The main idea is to transform extreme rays in extreme points of a suitable polytope. In this section we study three ways to normalize the dual subproblem described above.
 
 First, we note that the feasibility subproblem can be reformulated as a min cost flow problem in $\mathcal{N}^w$ with capacities $\boldsymbol{x}$ and arc costs $d_a$.
 \begin{align}
(NSP)^w \quad  \min\limits_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z},\boldsymbol{f}} & \quad \sum_{a\in A} d_a\, f_a & \\
\mbox{s.t. } & \quad \mbox{(\ref{flow_cons}), (\ref{Capacity}), (\ref{eq:nneg-f}).} & \nonumber %\\
%&\textbf{f}\ge 0& \nonumber
\end{align}
The associated dual subproblem is:
\begin{align}
(DNSP)^w \quad \max\limits_{\boldsymbol{\alpha},\boldsymbol{\sigma}} & \quad z\,\alpha_{w^s} - \sum_{e \in E} \sigma_e x_e \\
\mbox{s.t. } & \quad  \alpha_i - \alpha_j - \sigma_e \le d_a,& a=(i,j) \in A : e=\{i,j\}, \\
&\quad\sigma_e \ge 0,& e \in E.
\end{align}
Whenever $z^w>0$, the primal subproblem $(NSP)^w$ may be infeasible. Subproblems $(NSP)^w$ are no longer feasibility problems, although some of their respective dual forms can be unbounded. As the  splitting demand constraint has to be satisfied there are two kind of cuts to add:
\begin{enumerate}
 \item $(NSP)^w$ is infeasible and $(DNSP)^w$ is unbounded. In this case, the solution $(\boldsymbol{x},\boldsymbol{y},\boldsymbol{z})$ is cut by the constraint
 \begin{equation}
 \alpha_{w^s}\, z - \sum\limits_{e\in E}\sigma_e \, x_e \leq 0.
 \label{cut:norm1}
 \end{equation}
 \item $(NSP)^w$ is feasible and $(DNSP)^w$ has optimal solution. Consequently, if their solutions $(\boldsymbol{\alpha},\boldsymbol{\sigma})$ and $(\boldsymbol{x},\boldsymbol{y},\boldsymbol{z})$ satisfy that $\alpha_{w^s}\, z - \sum_{e\in E}\sigma_e \, x_e > u\, z$ then, the following cut is added
 \begin{equation}
 (\alpha_{w^s} - u)\, z - \sum\limits_{e\in E}\sigma_e \, x_e \leq 0.\label{cut:norm2}
 \end{equation}
\end{enumerate}



\noindent We refer to this implementation as \texttt{BD\_Norm1}. 

In this situation, there still exists dual subproblems $(DNSP)^w$ with extreme rays. We refer to \texttt{BD\_Norm2} as second dual normalization obtained by adding the dual constraint $\alpha_{w^s} = u + 1$. In this case, every extreme ray of $(SP)^w$ corresponds to one of the extreme points of $(NSP)^w$. A cut is added whenever the optimal dual objective value is positive. This cut has the following form:

\begin{equation}
z - \sum_{e \in E} \sigma_e\, x_e \le 0. \label{eq:normalized_cut} 
\end{equation}


We finally tested a third dual normalization, \texttt{BD\_Norm3}, by adding constraints
\begin{equation}
\sigma_e \leq 1,\qquad e \in E, \label{eq:normalized_cut2} 
\end{equation}
\noindent directly in $(DSP)^w$.


We tested the three dual normalizations described above for $(MC)$ using randomly generated networks with $10$, $20$ and $40$ nodes, as described in Subsection \ref{datasets}. As we will see in Section \ref{s:preliminary_results}, only \texttt{BD\_Norm1} results to be competitive.

\subsection{Facet-defining Benders cuts} \label{s:facertdef}

Here we describe how to generate Benders cuts for $(MC)$ based on the ideas exposed in \cite{Conforti2019facet}, named as $CW$. The procedure for $(PC)$ is the same. Given an \textit{interior point} or \textit{core point} $(\boldsymbol{x}^{in}, \boldsymbol{y}^{in}, \boldsymbol{z}^{in})$ of the convex hull of feasible solutions and an \textit{exterior point} $(\boldsymbol{x}^{out}, \boldsymbol{y}^{out}, \boldsymbol{z}^{out})$, that is a solution of the LP relaxation of the current restricted master problem, a cut that induces a facet or an improper face of the polyhedron defined by the LP relaxation of $Proj_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}\mathcal{F}(MC)$ is generated. We denote the difference $\boldsymbol{x}^{out} - \boldsymbol{x}^{in}$ by $\Delta \boldsymbol{x}$. We define $\Delta \boldsymbol{y}$ and $\Delta \boldsymbol{z}$ analogously. The idea is to find the furthest point from the core point, feasible to the LP-relaxation of $Proj_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}\mathcal{F}(MC)$ and lying on the segment line between the \textit{core point} and the \textit{exterior point}. This point is of the form $(\boldsymbol{x}^{sep}, \boldsymbol{y}^{sep}, \boldsymbol{z}^{sep}) = (\boldsymbol{x}^{out}, \boldsymbol{y}^{out}, \boldsymbol{z}^{out}) - \lambda (\Delta \boldsymbol{x}, \Delta \boldsymbol{y} , \Delta \boldsymbol{z})$. The problem of generating such a cut reads as follows:
\begin{align}
(SP\_CW)^w \quad \min_{\boldsymbol{f},\lambda} & \quad \lambda \\
\mbox{s.t. }& \quad \sum_{a \in \delta_w^+(i)} f_a -\sum_{a \in \delta_w^-(i)} f_a = 
 \begin{cases}
z^{out} - \lambda\,\Delta z, & \text{if $i = w^s$,}\\
0, & \text{otherwise,} 
\end{cases} \\
&\quad  f_a + f_{\hat{a}} \le x^{out}_e - \lambda\, \Delta x_e, \quad\qquad e=\{i,j\} \in E : a=(i,j), \hat{a}=(j,i),\\
& \quad \sum_{a \in A} d_a\, f_a \le u\,z^{out} - u\,\Delta z\, \lambda, \\
&\quad  0\le \lambda \le 1, \\
&\quad  f_a \ge 0,\hspace{8cm} a \in A.
\end{align}
In order to obtain the Benders feasibility cut we solve its associated dual:
\begin{align}
(DSP\_CW)^w \quad \max_{\boldsymbol{\alpha}, \boldsymbol{\sigma},\boldsymbol{\upsilon}} &\quad z^{out}\,\alpha_{w^s} - \sum_{e \in E} x^{out}_e\,\sigma_e - u\,z^{out}\, \upsilon \\
\mbox{s.t. }&\quad \Delta z\, \alpha_{w^s} - \sum_{e \in E} \Delta x_e\,\sigma_e - u\, \Delta z\, \upsilon \le 1, \label{eq:normcw}\\
&\quad \alpha_i - \alpha_j -\sigma_e - d_a\,\upsilon \le 0,\qquad\qquad\quad a=(i,j) \in A : e=\{i,j\},\nonumber\\
&\quad \sigma_e,\,\upsilon\ge 0, \hspace{6.9cm} e\in E. \nonumber
\label{sub:CW}
\end{align}
Given that $(SP\_CW)^w$ is always feasible ($\lambda = 1$ is feasible) and that its optimal value is lower bounded by 0, then, both $(SP\_CW)^w$ and $(DSP\_CW)^w$ have always finite optimal solutions. Whenever the optimal value of $\lambda$ is 0, $(\boldsymbol{x}^{out}, \boldsymbol{y}^{out}, \boldsymbol{z}^{out})$ is feasible. A cut is added if the optimal value of $(DSP\_CW)^w$ is strictly greater than 0. The new cut has the same form as in (\ref{eq:feasibility_cut}). Note that this problem can be seen as a dual normalized version of $(SP)^w$ with the dual constraint \eqref{eq:normcw}. This approach is an improvement in comparison with the stabilization cuts proposed by \cite{ben2007acceleration}, where $\lambda$ is a fixed parameter.

Core points for both formulations can be obtained by computing the average of the points described in the proof of Proposition \ref{prop_MC} for $(MC)$ and the average of the points in list $L$ obtained by applying Algorithm~\ref{pre_2}.

\subsection{Cut-set inequalities} \label{s:cutset}

By projecting out variable vector $\boldsymbol{f}$, information regarding the link between vectors $\boldsymbol{x}$ and $\boldsymbol{z}$ is lost. {\it Cut-set inequalities} represent the information lost regarding the connectivity for the O/D pair $w$ in the solution given by the design variable vector $\boldsymbol{x}$. Let $(S,S^C)$ be a $(w^s,w^t)$-partition of $N^w$ for a fixed O/D pair $w$, i.e. $(S,S^C)$ satisfies: i. $w^s\in S$; ii. $w^t \in S^C$, with $S^C=N\setminus S$ its complement. A {\it cut-set inequalities} is defined as
\begin{equation}
z^w \leq \sum_{\substack{\{i,j\} \in E^w: \\ i\in S, \, j \in S^C}} x_{\{i,j\}}, \quad w \in W,\quad (S,S^C) \mbox{ a } (w^s,w^t)\mbox{-partition of } N^w. \label{eq:cutset}
\end{equation}
\noindent This type of constraints has been studied in several articles, for instance \cite{Barahona1996network,Koster2013extended, Costa2009benders}. Note that it is easy to see that cut-set inequalities belong to the LP-based Benders family. Let $(S,S^C)$ be a $(w^s,w^t)$-partition in the graph $\mathcal{N}^w$ for $w\in W$. Consider the following dual solution:

\begin{itemize}
	\item $\alpha_i = 1$ if $i\in S$; $\alpha_i = 0$ if $i\in S^C$.
	\item $\sigma_e=1$ if $e=\{i,j\} \in E^w$, $i\in S$, $j \in S^C$; $\sigma_e=0$, otherwise.
	\item $\upsilon = 0$.
\end{itemize}

This solution is feasible to $(DSP)^w$ and induces a cut as in (\ref{eq:cutset}). In order to improve computational performance, we test two approaches to include these inequalities:

\begin{enumerate}
	\item We implement a modification of the Benders callback algorithm with the following idea. First, for each $w\in W$, using the solution vector $(\boldsymbol{x},\boldsymbol{y})$ from the master, the algorithm generates a network $(N^w,E^w)$ with capacity $1$ for each edge built. Then, a \textit{Depth-First Search (DFS)} algorithm is applied to obtain the connected component containing $w^s$. If the connected component does not contain $w^t$, a cut of the form (\ref{eq:cutset}) is added. Otherwise, we generate a Benders cut as before. This routine is depicted in Algorithm \ref{cut_set_implment}.

	\begin{algorithm}[htpb] 
		\caption{Callback implementation with cut-set inequalities.} 
		\label{cut_set_implment} 
		\begin{algorithmic} 
			\REQUIRE ($x_e, e\in E$, $z^w, w\in W$) from the master solution solution $(\boldsymbol{x},\boldsymbol{y},\boldsymbol{z})$.
			\FOR{$w \in W$}
				\STATE Build graph $(N^w({\boldsymbol x}),E^w({\boldsymbol x}))$ induced by the solution vector $\boldsymbol{x}$ from the master.
					
				\STATE Compute the connected component $S$ in $(N^w({\boldsymbol x}),E^w({\boldsymbol x}))$ containing $w^s$.
				\IF{$w^t$ is not included in $S$}
					\STATE Add the cut $
							z^w \leq \sum_{\substack{\{i,j\} \in E^w: \\ i\in S, \, j \in S^C}} x_{\{i,j\}}
							$
				\ELSE
					\STATE Solve the corresponding subproblem ($(DSP)^w$, $(DNSP)^w$, $(DSP\_CW)^w$) and add cut if it is necessary.
				\ENDIF
				\ENDFOR
			\RETURN Cut.
		\end{algorithmic}\label{algorithm:3}
	\end{algorithm}
	
	
We tested this implementation with subproblems $(DSP\_CW)^w$. We observe that by using Algorithm \ref{algorithm:3} with $CW$ the convergence is slower and we generate more cuts. These preliminary results are shown in Table \ref{t:pre_res_cs}. 
 

 	
	\item We add to the \textit{Master Problem} the \textit{cut-set inequalities} at the origin and at the destination of each O/D pair $w\in W$ at the beginning of the algorithm. These valid inequalities have the form:
	
	\begin{gather}
	\begin{cases}
	z^w \leq \sum\limits_{e \in \delta(w^s)} x_e ,\\
	z^w \leq \sum\limits_{e \in \delta(w^t)} x_e .
	\end{cases}\label{eq:cutset2}
	\end{gather}
	
	
	This means that for each O/D pair to be covered, there should exist at least one edge incident to its origin and one edge incident to its destination, i.e. each O/D pair should have at least one arc going out of its origin and another one coming in its destination.
\end{enumerate}



==> paper Benders Decomposition draft ArXiv - tercera versi�n/biblio.tex <==
\begin{thebibliography}{1}


\bibitem{Balas2002}%balas2002lift
E. Balas and  M. Perregaard. Lift-and-project for Mixed 0–1 programming: recent progress. \textit{Discrete Applied Mathematics}, 123(1-3), 129–154, 2002. 
% https://doi.org/10.1016/S0166-218X(01)00340-7

\bibitem{Balas2003}%balas2003precise
E. Balas and  M. Perregaard. A precise correspondence between lift-and-project cuts, simple disjunctive cuts, and mixed integer gomory cuts for 0-1 programming. \textit{Mathematical Programming}, 94(2-3), 221–245, 2003. 
% https://doi.org/10.1007/s10107-002-0317-y

\bibitem{Barahona1996network}
 F. Barahona. Network Design Using Cut Inequalities. \textit{SIAM Journal on Optimization}, 6(3), 823–837, 1996.
% https://doi.org/10.1137/S1052623494279134

\bibitem{Ben2007acceleration}
W. Ben‐Ameur, J. Neto, L. Gouveia, and S. Voss. Acceleration of cutting‐plane and column generation algorithms: Applications to network design. \textit{Networks}, 49(1), 3–17, 2007.
% https://doi.org/10.1002/net.20137

\bibitem{Ben1962}%Ben
J. F. Benders. Partitioning procedures for solving mixed-variables programming problems. \textit{Numerische Mathematik}, {\bf
4}, 232--252, 1962.

\bibitem{Berge1957}
C. Berge. Two theorems in Graph Theory.  \textit{Proceedings of the National Academy of Sciences of the United States of America}, {\bf 43(9)} 842--844, 1957.

\bibitem{Berman2009}%BDKW
O. Berman , Z. Drezner, D. Krass and G.O. Wesolowski. The variable radius covering problem. \textit{European Journal of Operational Research}, {\bf 196}, 516--525, 2009.

\bibitem{Canca2017}%CDLM17
D. Canca, A. De-los-Santos, G. Laporte and J. A. Mesa. An adaptive neighborhood search metaheuristic for the integrated
rapid transit network design and line planning problem, \textit{Computers \& Operations Research}, {\bf 78}, 1--14, 2017.


\bibitem{Canca2019}%CDLM19
D. Canca, A. De-los-Santos, G. Laporte and J. A. Mesa. Integrated railway rapid transit network design and line planning problem with maximum profit, \textit{Transportation Research Part E: Logistics and Transportation Review}, {\bf 127}, 1--30, 2019.

\bibitem{Cascetta2009}%Cas
E. Cascetta. \textit{Transportation System Analysis: Models and Applications}, Springer, 2009.

\bibitem{Church2018}%ChMu
 R. Church and A. Murray. \textit{Location Covering Models}, Springer, 2018.
 
\bibitem{Church1974}%ChRe
R. Church and C. ReVelle. The maximal covering location problem. \textit{Papers of the Regional Science Association}. {\bf 32}, 101--118, 1974.

\bibitem{Conforti2019facet}
M. Conforti and L. Wolsey. “Facet” separation with one linear program. \textit{Mathematical Programming}, 178(1), 361–380, 2019.
% https://doi.org/10.1007/s10107-018-1299-8

\bibitem{Cordeau2019benders}
J. F. Cordeau, F. Furini and I. Ljubić. Benders decomposition for very large scale partial set covering and maximal covering location problems. \textit{European Journal of Operational Research}, 275(3), 882-896, 2019.

\bibitem{Costa2009benders}
A. Costa, J. Cordeau and B. Gendron. Benders, metric and cutset inequalities for multicommodity capacitated network design. \textit{Computational Optimization and Applications}, 42(3), 371–392, 2009.

\bibitem{Desrochers1988algorithm}
Martin Desrochers. \textit{An algorithm for the shortest path problem with resource constraints}, {\'E}cole des hautes {\'e}tudes commerciales, Groupe d'{\'e}tudes et de recherche en analyse des décisions, 1988.


\bibitem{Farahani2012}%FAHHG
R. Z. Farahani, N. Asgari, N. Heidari, M. Hosseininia and M. Goh. Covering problems in facility location: a review. \textit{Computers and Industrial Engineering}, {\bf 62} 368--407, 2012.

\bibitem{Fischetti2010note}
M. Fischetti, D. Salvagnin and A. Zanette. A note on the selection of Benders’ cuts. \textit{Mathematical Programming}, 124(1-2), 175–182, 2010.

\bibitem{Garcia2013}%GaLMP
B. García-Archilla, A. J. Lozano, J. A. Mesa and F. Perea. GRASP algorithms for the robust railway network design problem. \textit{Journal of Heuristics}, {\bf 19}, 399--422, 2013.

%\JAM{
% \bibitem{GarciaMarin2020} 
% S. García, A. Marín. Covering Location Problems,

\bibitem{Hakimi1965}%Hak
S. L. Hakimi. Optimum distribution of switching centers in a communication network and some related graph theoretic problems.
\textit{Operations  Research}, {\bf 13}, 462--475, 1965.

\bibitem{Hakimi1993}
S. L. Hakimi, E. F. Schmeichel and M. Labbé. On locating path‐or tree‐shaped facilities on networks. \textit{Networks}, 23(6), 543-555, 1993.

\bibitem{Johnson1978}%JLR
D. S. Johnson, J. K. Lenstra and A. H. G. Rinooy Kan. The complexity of the network design problem, \textit{Networks}, {\bf 8}, 279--285, 1978.

\bibitem{Karp1971}%Karp
R. M. Karp. Reducibility among combinatorial problems. \textit{Complexity of Computers Computations} (R. E. Miller, J. W. Tatcher, J. D. Bohlinger, eds.), 85--103, Plenum, New York, 1971.

\bibitem{Koster2013extended}
A. Koster, T. Phan and M. Tieves. Extended Cutset Inequalities for the Network Power Consumption Problem. \textit{Electronic Notes in Discrete Mathematics}, 41(C), 69–76, 2013.

\bibitem{Krol2019}%KK
 A. Król and M. Król. The design of a metro network using a genetic algorithm. \textit{Applied Science}, 9, 433, 2019.

\bibitem{Ljubic2012exact}
I. Ljubić, P. Putz and J. Salazar‐González. Exact approaches to the single‐source network loading problem. \textit{Networks}, 59(1), 89–106, 2012.

\bibitem{Magnanti1986}%MagMirWong 
T. L. Magnanti, P. Mireault and R. T. Wong. Tailoring Benders decomposition for uncapacitated network design. \textit{Netflow at Pisa}. Mathematical Programming Studies (G. Gallo, C. Sandi, eds.), vol 26, Springer, Berlin, Heidelberg, 1986.

\bibitem{Magnanti1981accelerating}
T. L. Magnanti and R. T. Wong. Accelerating Benders Decomposition: Algorithmic Enhancement and Model Selection Criteria. \textit{Operations Research}, 29(3), 464–484, 1981.

\bibitem{Magnanti1984}%MagWong
T. L. Magnanti and R. T. Wong. Network Design and Transportation Planning: Models and Algorithms. \textit{Transportation Science}, {\bf 18}, 1--55, 1984.


\bibitem{Marin2009}%MJ
A. Marín and P. Jaramillo. Urban rapid transit network design: acceleraded Benders decomposition. \textit{Annals of Operations Research}, {\bf
169} 35--53, 2009.

\bibitem{Melkote2001}%MelDas
S. Melkote and M. S. Daskin. An integrated model of facility location and transportation network design. \textit{Transportation Research, Part A}, {\bf 35}, 515--538, 2001.

\bibitem{Mesa2018}
J. A. Mesa. Comments: on Extensive facility location on networks: an updated review 1. \textit{TOP}, {\bf 6(2)}, 227--228, 2018.

\bibitem{Mesa1991}%MeBo
J. A. Mesa and B. T. Boffey.  A review of extensive facility location in networks. \textit{European Journal of Operational Research} {\bf 95}, 592--603, 1991.

\bibitem{Norman1959}%NorRa
R. Z. Norman and M. O. Rabin. An algorithm for a minimum cover of a graph. \textit{Proceedings of the American Mathematical Society}, {\bf 10}, 315--319, 1959.

\bibitem{Perea2020}%PMMR
F. Perea, M. Menezes, J. A. Mesa and F. Rubio-del-Río. Transportation infrastructure network design in presence of modal competition: computational complexity classification and a genetic algorithm. \textit{TOP}, {\bf 28}, 442--474, 2020.

\bibitem{Puerto2018}%PRS
J. Puerto, F. Ricca and A. Scozzari. Extensive facility location on networks: and updated review. \textit{TOP}, {\bf 6(2)}, 187-226, 2018.

\bibitem{Rahmaniani2017}%RCGR
R. Rahmaniani, T. G. Crainic, M. Gendreau and W. Rei. The Benders decomposition algorithm: A literature review. \textit{European Journal of
Operational Research}, {\bf 259} 801--817, 2017.


\bibitem{Schilling1993}%SchJaBar
D. A. Schilling, V. Jayamaran and R. Barkhi. A review of covering problems in facility location. \textit{Location Science}. {\bf 1}, 25--55, 1993.

\bibitem{sioux}
Sioux Networks, \url{http://www.bgu.ac.il/~bargera/tntp/SiouxFalls_CNDP/SiouxFallsVariantsForNetworkDesign.html}


\bibitem{Toregas1971}%TSRB
C. Toregas, R. Swain, C. ReVelle and L. Bergman. The location of emergency services facilities.
\textit{Operations Research}, {\bf 19}, 1363--1373, 1971.

\bibitem{FORTZ2009359}%TSRB
B. Fortz and M. Poss. An improved Benders decomposition applied to a multi-layer network design problem
\textit{Operations Research Letters}, {\bf 37}, 359 -- 364, 2009.

\bibitem{botton2013benders}%TSRB
Botton, Quentin and Fortz, Bernard and Gouveia, Luis and Poss, Michael. Benders decomposition for the hop-constrained survivable network design problem.
\textit{INFORMS journal on computing}, {\bf 25}, 13--26, 2013.

\bibitem{schmidt2014location}%TSRB
Schmidt, Marie and Sch{\"o}bel, Anita. Location of speed-up subnetworks.
\textit{Annals of Operations Research}, {\bf 1}, 379--401, 2014.


\end{thebibliography}

==> paper Benders Decomposition draft ArXiv - tercera versi�n/literature.tex <==

%Covering problems in graphs have attracted the attention of
%researchers since the middle of last century. As far as the
%authors are aware the first papers on the vertex-covering problem
%were due to Berge \cite{Berge1957} and Norman and Rabin \cite{Norman1959} in the latest 50s. This problem is related with the set-covering problem in which a family of sets is given and the minimal subfamily \ML{whose} union contains all the elements is sough \ML{for}.
% The decision versions of both problems were  proved to be NP-complete \cite{Karp1971}. In \cite{Hakimi1965} the vertex-covering problem was formulated as an integer linear programming model and solved by
%using Boolean functions.

%Authors in \cite{Toregas1971} applied the vertex-covering problem to the location of emergency services. They assumed that a vertex is covered if it is within a given coverage distance. Church and ReVelle introduced the maximal covering location problem by fixing the number of facilities to be located \cite{Church1974}. Each vertex has an associated population and the objective is to cover the maximum population within a fixed distance threshold. Since then many variants and extensions of the vertex-covering and maximal covering  problems have been
%researched (see \cite{Schilling1993}, \cite{Berman2009}, \cite{Farahani2012}, \cite{Church2018}, and the references therein).

%An  extensive facility location problem consists of locating a subgraph such as to optimize some objective function with some contraints regarding demand points \cite{Mesa1991}, \cite{Puerto2018}. Problems where a path or a tree-graph with a possibly  limited length so that the maximum distance or the sum of distances to the vertices is minimized generalize, to non-point
%facilities, the concept of center and median,  respectively. In these papers extensive location problems with other
%objective functions as k-centrum, ordered median and equity
%measures have also been reviewed. Several papers have dealt with
%extensive facility location with covering objectives (see \cite{Mesa2018}, and the references therein). The extensive vertex-covering and maximal covering problems are extensions of the point vertex-covering and maximal covering problems where the number
%of vertices of the coverage is substituted by the length or other characteristic of the covering subgraph.
%These problems depend on the type of underlying graph, the location of the demand, the shape of the graph used for covering and its tips (discrete or continuous), the way of covering and other characteristics. Indirect and direct covering of a graph by a subtree with limited number of vertices or bounded length problems are NP-hard in general, since they are special cases of the Steiner tree problem. However, if the underlying graph is a tree some of the problems can be solved by polynomial time algorithms, those cases in which paths are being sought \cite{Hakimi1993}. If the search consists of a tree there are some NP-hard problems, among which stands out Median Problem.

%Network design is a broad and spread subject whose models often depend on the field in which they are applied. However, a systematization was done by authors in \cite{Magnanti1984} where some classical graph problems as the minimal spanning tree, Steiner tree, shortest path and traveling salesman problems
 %are included as particular cases of a general mathematical programming model.
 %Discrete network design problems assume that a given underlying graph is given,
 %and could  be classified into four groups with increasing complexity: without capacity, with capacity, capacity or coverage expansion, and multiperiod. Extensive facility location and network design are interlaced subjects where synergies often appear. Moreover, network design and point-location problems are
 %very related since the transportation network is the way to access the facilities and, therefore the efficiency of the optimal point depends on the network design. In fact several models integrate the location of facilities and the design of the network used to fulfill the demand. The objective function of the model in \cite{Melkote2001} includes transportation cost, facility location, and construction of the network. However, very early was stated the NP-hardness of a special network design problem. Authors in \cite{Johnson1978} showed that the knapsack problem is reducible to the problem of choosing a subgraph that minimizes the sum of the shortest path weights between all vertex pairs subject to a budget constraint.

%All the previously reviewed research considers a
%customer-to-server system, where demand uses the network to access
%the point or extensive facilities. However, in many cases reaching
% or been closed to a facility is not enough to complete the
%service. In many telecommunication, transportation, public
%services  and other systems the demand uses the facility as an
%intermediate instead of a final step. 

%For example, this is the case of public urban transportation network where a customer have to spend time to reach the stop/station from its origin, then
%wait for the next service, spend  in-vehicle time, and finally
%reach its destination. Network design of these systems are even
%more complex than those where the customers have just to go to the
%servers.

%In these cases the demand is given by pairs instead of
%points, and usually each pair has an associated weight indicating
%the traffic between the origin and the destination. Usually this
%demand is encoded using an origin-destination matrix. When planning a new network, often there exists a network already functioning and
%offering its service to the same set of origin-destination pairs.
%For example, in order to improve the mobility of a big city or
%metropolitan area, a new rapid transit systems is planned. The
%current transit system could be more dense than the rapid transit
%planned but slower since uses the same right-of-way than the
%private traffic. Thus, in some way both systems compete between
%them and both compete with the private mode of transportation.
%A similar effect occurs with mobile telecommunication operators. 
%Therefore, the traffic between an origin and a destination is distributed among the several systems that provide the service. 

%There are mainly two ways of allocating the share of each mode. The first one is the binary all-or-nothing way, where the demand is served by each mode only if the mode the demand point within a range of quality service, as in \cite{church1974maximal}. The second one is some continuous function, for example multi-logit probability distributions, as in \cite{cascetta2009transportation}. Both mode-share are based in the comparison of distances, times, costs, generalized costs or utilities. In this paper,  we consider a binary one, where each pair is served only if the time spent into the network is below a threshold. This threshold represents the comparison between the time spent in the proposed network and a private mode assigning the full share to the most beneficial one. When the aim is to maximize the sum of the
 %weights of the covered pairs by the new network, and the constraint is the total cost of the network the problems of finding an optimal network without cycles and allowing cycles are NP-Hard \cite{perea2020transportation}. 
 
 Since most network design problems are NP-hard,  recent research efforts have been oriented to apply metaheuristic algorithms to obtain good solutions in a reasonable computational time. Thus, in the field of transportation network design, Genetic Algorithms (\cite{krol2019design}), Greedy Randomized Adaptive Search Procedures
 (\cite{garcia2013grasp}),  Adaptive Large Neighborhood Searchs  (\cite{canca2017adaptive}) and
  metaheuristics (\cite{canca2019integrated}) have been applied to rapid transit network design problems with applications to medium-size instances.  
  
  In this article we propose exact methods based on Benders' decomposition. Benders proposed this decomposition for solving mixed-integer mathematical programming problems in the early 60s \cite{benders2005partitioning}. Since then, it has been applied to many problems in different fields, see \cite{rahmaniani2017benders}  for a recent literature review on the use of Benders decomposition in combinatorial optimization. One remarkable recent contribution applied to set covering and maximal covering location problems  appears in \cite{Cordeau2019benders}.

 Benders decomposition for network design problems have been studied since the 80s. In \cite{magnanti1986tailoring}, authors minimize the total building cost of an uncapacitated network subject to the constraints that all O/Ds pairs must be served. Given the structure of the problem, the Benders reformulation is stated with one sub-problem for each pair O/D. A Benders decomposition for a multi-layer network design problem is 
presented in \cite{FORTZ2009359}. Benders decomposition were also applied in \cite{botton2013benders} in the context of designing survivable networks. Authors in \cite{Costa2009benders} have studied multi-commodity capacitated network design and the strength of different Benders cuts; in \cite{marin2009urban} a multi-objective approach is solved through Benders decomposition where coverage is maximized, but at the same time total cost design is minimized. To best of our knowledge, this is the first time that a branch-and-Benders-cut approach is applied to network design coverage problems. We also study for the first time in this context the inclusion of {\it facet-defining cuts} as was recently proposed by \cite{Conforti2019facet}.


==> paper Benders Decomposition draft ArXiv - tercera versi�n/literature_JA.tex <==

Covering problems in graphs have attracted the attention of
researchers since the middle of last century. As far as the
authors are aware the first papers on the vertex-covering problem
were due to Berge (1957)  \cite{Berge} and Norman and Rabin (1959) \cite{NorRa}  The problem
dealt with in these papers was to find a subset of vertices with
minimum cardinality such that each edge is incident to at least
one vertex of it. This problem is related with the set-covering problem in which a family of sets is given and the minimal subfamily which union contains all the elements is sough.
Current file
Overview
2

 The decision versions of both problems were  proved to be   NP-complete (Karp (1972) \cite{Karp}). The
 vertex-covering problem was formulated as an integer linear programming model and solved by
using Boolean functions by Hakimi (1965)  \cite{Hak}.
This problem was applied to the location of emergency services by
Toregas et al. (1971) \cite{TSRB}. They assumed a vertex is
covered by other if they are within a given coverage distance. When the number of facilities
to be located is fixed then the maximal covering location problem
arises (Church and ReVelle, (1974) \cite{ChRe})  in which problem each vertex has an
 associated population and the objective is to cover the maximum
population within a fixed distance threshold. Since then many
variants and extensions of the vertex-covering and maximal covering  problems have been
researched (see, Schilling et al., (1993) \cite{SchJaBar}, Berman et al., (2009) \cite{BDKW},
Farahani et al. (2012) \cite{FAHHG}, and  Church and Murray, (2018) \cite{ChMu}, and the references therein).

An  extensive
facility location problem consists of locating a subgraph such
that optimizes some objective function with some contraints regarding demand points
(see, Mesa and Boffey, 1991 \cite{MeBo}, and Puerto et al.  (2018) \cite{PRS}.) Problems where a
path or a tree-graph with a possibly  limited length so that the maximum
distance or the sum of distances to the vertices is minimized
generalize,  to non-point
facilities, the concept of center and median,  respectively. In these papers extensive location problems with other
objective functions as k-centrum, ordered median and equity
measures have also been reviewed. Several papers have dealt with
extensive facility location with covering objectives (see, Mesa,
(2018) \cite{Mesa}, and the references therein). The extensive vertex-covering and maximal covering problems are extensions of the point vertex-covering and maximal covering problems where the number
of vertices of the coverage is substituted by the length or other characteristic of the covering subgraph.
The problems depend on the type of underlying graph, the location of the demand, the shape of the graph used for covering and its tips (discrete or continuous), the way of covering and other parameters.
Indirect and direct covering of a graph by a subtree with
limited number of vertices or bounded length problems are
 NP-hard in general, since they are special cases of the Steiner tree problem.
 However, if the underlying graph is a tree most of the problems can be solved by  polynomial time algorithms.

Network design is a broad and spread subject whose models often depend on the field in which they are applied. However,
a systematization was done by Magnanti and Wong (1984) \cite{MagWong}
where some classical graph problems as the minimal spanning tree, Steiner tree, shortest path and traveling salesman problems
 are included as a particular cases of a general mathematical programming model.
 Discrete network design problems assume that a given underlying graph is given,
 and could  be classified into four groups with increasing complexity: without capacity, with capacity,
 capacity or coverage expansion, and multiperiod. Extensive facility location and network design are
 interlaced subjects where synergies often appear. Moreover, network design and point-location problems are
 very related since the transportation network is the way to access the facilities and, therefore the efficiency of the optimal point depends on the network design. In fact several relatively recent models integrate the location of facilities and the design of the network used to fulfill the demand. The objective function of the model in the paper by Melkote and Daskin (2001) \cite{MelDas} includes transportation cost, facility location, and construction of the
 network. However, very early was stated the NP-hardness of a
 special network design problem. In the paper by Johnson et al. (1978) \cite{JLR}, it was shown that the knapsack problem is reducible to the problem of choosing a subgraph such that it minimizes the sum  of the shortest path weights between all vertex pairs subject to a budget constraint.

All the previously reviewed research considers a
customer-to-server system, where demand uses the network to access
the point or extensive facilities. However, in many cases reaching
or been closed to a facility is not enough to complete the
service. In many telecommunication, transportation, public
services  and other systems the demand uses the facility as an
intermediate instead of a final step. This is, for example, the
case of public urban transportation network, where a customer have
to spend  a time to reach the stop/station from its origin, then
wait for the next service, spend an in-vehicle time, and finally
reach its destination. Network design of these systems are even
more complex than those where the customers just have to go to the
servers. 

In this cases the demand is given by pairs instead of
points, and usually each pair has an associated weight indicating
the traffic between the origin and the destination. Usually this
demand is codify by an origin-destination matrix. When planning a
new network, often there exists a network already functioning and
offering its service to the same set of origin-destination pairs.
For example, in order to improve the mobility of a big city or
metropolitan area, a new rapid transit systems is planned. The
current transit system could be more dense than the rapid transit
planned but slower since uses the same right-of-way than the
private traffic. Thus, in some way both systems compete between
them and both compete with the private mode of transportation.
 Almost the same happens with mobile telecommunication operators. Therefore, the traffic between an origin and
 a destination is distributed among the several systems that provide the service. There are mainly two ways of
 allocating the share of each mode. The first one is the binary  all-or-nothing, the second one is some continuous
 function (see Cascetta, 2009, \cite{Cas}). Both mode-share are based in the comparison of distances, times, costs,
 generalized costs or utilities. The second is more for real but, in this paper,  we will use the binary one.
 Since the main aim of this paper is not to have a good representation of the reality but to assess the Benders'
 decomposition in a basic planning infrastructure network design, we will use the binary distribution.
 For this purpose, usually the utility of both modes are compared for each  o-d pair and  is assigned the
 share one to the most beneficial  and zero to another.  When the aim is to maximize the sum of the
  weights of the covered pairs by the new network, and the constraint is the total cost of the network the problems of finding
  an optimal network without cycles and allowing cycles are NP-Hard (Perea et al. (2020),
  \cite{PMMR}).Since most of the network design problems are
  NP-hard, the recent research efforts have been oriented to apply
  metaheuristic algorithms to obtain good solutions in a
  reasonable computational time. Thus, in the field of
  transportation network design, Genetic Algorithms (Król amd
  Król, (2019), \cite{KK}), Greedy Randomized Adaptive Search Procedure
  (Garc\'\i a-Archilla et al., 2013, \cite{GaLMP}),  Adaptive Large
  Neighborhood Search (Canca et al. 2017, \cite{CDLM17}) and
  matheuristic (Canca et al. 2019, \cite{CDLM19}) have been applied
  to rapid transit network design problems with applications to
  medium-size instances. Although exact methods cannot solve
  nowadays large instances in a short time, infrastructure network
  design problems belong to the strategic phase of the sequential
  process of transportation planning and, therefore, computational
  time is less important than to other problems belonging to
  operational or on-line phases. Moreover, exact methods require a
  more profound knowledge, and thus provide more insight on the
  problems and mathematical models. Benders decomposition was
  proposed by Benders (1962, \cite{Ben}) for solving mixed-integer
  mathematical programming problems. Since then, it has been
  applied to many problems in different fields, see \cite{RCGR}
  for a recent literature review on the use of Benders
  decomposition in combinatorial optimization. One remarkable recent contribution appears in \cite{cordeau2019benders} in the context of set covering and maximal covering. 

 Benders decomposition for network design problems have been studied since the 80s. In \cite{MagMirWong}, authors minimize the total building cost of an uncapacitated network subject to the constraints that all O/Ds pairs must be served. Given the structure of the problem, the Benders reformulation is stated with one sub-problem for each pair O/D. Authors in \cite{costa2009benders} studied multicommodity capacitated network design and study the strength of different Benders cuts; in \cite{MJ} a multi-objective approach is solved through Benders decomposition where coverage is maximized, but at the same time total cost design is minimized. To best of our knowledge, this is the first time that a branch-and-Benders-cut approach is applied to network design coverage problems. We also study for the first time in this context the inclusion of {\it facet-define cuts} as it was recently proposed by \cite{conforti2019facet}.

==> paper Benders Decomposition draft ArXiv - tercera versi�n/models.tex <==
\section{Problem formulations and some properties}\label{s:models}
In this section we present mixed integer linear formulations for the Maximal Covering Network Design Problem $(MC)$ and the Partial Set Covering Network Design Problem $(PC)$. We also describe some pre-processing methods and finish with some polyhedral properties. We first introduce some notation.

We consider an undirected graph denoted by $\mathcal{N} = (N,E)$, where $N$ and $E$ are the sets of potential nodes and edges that can be constructed. Each element $e \in E$ is denoted by $\{i,j\}$, with $i,j \in N$. We use the notation $i\in e$ if node $i$ is a terminal node of $e$. Let $\delta(i)$ be the set of edges incident to node $i$.

The mobility patterns are represented by a set $W\subset N\times N$ of O/D pairs. Each $w = (w^s,w^t)\in W$ is defined by an origin node $w^s \in N$, a destination node $w^t\in N$, an associated demand $g^w > 0$ and a utility $u^w > 0$. This utility translates the fact that there already exists a different network competing with the network to be constructed in an all-or-nothing way. In other words, an O/D pair $(w^s,w^t)$ will travel on the newly constructed network if it contains a path between $w^s$ and $w^t$ of length shorter than or equal to the utility $u^w$. We then say that the O/D pair is covered. In terms of the transportation area, the existing network represents a private transportation mode, the planned one represents a public transportation mode and the parameter $u^w,\,w\in W$, refers to the utility of taking the private mode.

Costs for building nodes, $i\in N$, and edges, $e \in E$, are denoted by $b_i$ and $c_e$, respectively. The total construction cost cannot exceed the budget $C_{max}$. For example, in the context of constructing a transit network, each node cost may represent the total cost of building one station in a specific location in the network. On the other hand, each edge cost represents the total cost of linking two stations. 

For each $e=\{i,j\}\in E$, we define two arcs: $a=(i,j)$ and $\hat{a} =(j,i)$. The resulting set of arcs is denoted by $A$. The length of arc $a \in A$ is denoted by $d_a$. For each O/D pair $w \in W$ we define a subgraph $\mathcal{N}^w = (N^w, E^w)$ containing all feasible nodes and edges for $w$, i.e. that belong to a path in $\mathcal{N}$ whose total length is lower than or equal to $u^w$. We also denote $A^w$ as the set of feasible arcs. In Section \ref{s:pre}, we describe how to construct these subgraphs. We use notation $\delta_w^+(i)$ ($\delta_w^-(i)$ respectively) to denote the set of arcs going out (in respectively) of node $i \in N^w$. In particular, $\delta_w^-(w^s) = \emptyset$ and $\delta_w^+(w^t) = \emptyset$. We also denote by $\delta_w(i)$ the set of edges incident to node $i$ in graph $\mathcal N^w$.


\subsection{Mixed Integer Linear Formulations}\label{s:formulations}

We first present a formulation of the \textit{Maximal Covering Network Design Problem} $(MC)$, whose aim is to design an infrastructure network maximizing the total demand covered subject to a budget constraint: 

\begin{align}
(MC) \quad \max_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z},\boldsymbol{f}} &\quad \sum_{w \in W} g^w z^w &\label{eq:MCobj}\\ 
\mbox{s.t. } &\quad \sum_{e \in E} c_e x_e + \sum_{i \in N} b_i y_i \le C_{max}, \label{eq:budget} \\
&\quad x_e \le y_i,\hspace{8cm} e \in E, i \in e, \label{rel_xy}\\
&\quad \sum_{a \in \delta_w^+(i)} f^w_a -\sum_{a \in \delta_w^-(i)} f^w_a = 
 \begin{cases}
z^w, &\text{if $i = w^s$},\\
-z^w, &\text{if $i = w^t$}, \\
0, & \text{otherwise}, 
\end{cases} \hspace{1.8cm} w \in W, i \in N^w, \label{flow_cons}\\
&\quad f^w_{a}+f^w_{\hat{a}} \le x_{e}, \hspace{2cm} w \in W,\, e=\{i,j\} \in E^w: a=(i,j), \, \hat{a}=(j,i),\label{Capacity} \\
&\quad \sum_{a \in A^w} d_a f^w_a \le u^w z^w, \hspace{7cm} w \in W, \label{Utility} \\
&\quad y_i,\, x_e,\, z^w \in \{0,1\}, \hspace{5cm} i\in N,\, e\in E,\, w\in W,\label{eq:nat}\\ 
&\quad f_a^w \in \{0,1\}, \hspace{7cm} a \in A^w, w\in W,\label{eq:nat-f}
\end{align}
\noindent where $y_i$ and $x_e$ represent the binary design decisions of building node $i$ and edge $e$, respectively. Mode choice variable $z^w$ takes value $1$ if the O/D pair $w$ is covered and $0$ otherwise. Variables $f_a^w$ are used to model a path between $w^s$ and $w^t$, if possible. Variable $f_a^w$ takes value $1$ if arc $a$ belongs to the path from $w^s$ to $w^t$, and $0$ otherwise. Each variable $f^w_a$, such that $a\notin A^w$, is set to zero.

The objective function (\ref{eq:MCobj}) to be maximized represents the demand covered. Constraint (\ref{eq:budget}) limits the total construction cost. Constraint (\ref{rel_xy}) ensures that if an edge is constructed, then its terminal nodes are constructed as well. For each pair $w$, expressions (\ref{flow_cons}), (\ref{Capacity}) and (\ref{Utility}) guarantee demand conservation and link flow variables $f_a^w$ with decision variables $z^w$ and design variables $x_e$. Constraints (\ref{Capacity}) are named capacity constraints and they force each edge to be used only in one direction at most. Constraints (\ref{Utility}) referenced as mode choice constraints, put an upper bound on the length of the path for each pair $w$. This ensures variable $z^w$ to take value $1$ only if there exists a path between $w^s$ and $w^t$ with length at most $u^w$. This path is represented by variables $f_a^w$. %From the bilevel optimization point of view, this is an optimistic assumption because in case of ties the user will choose the solution with maximal coverage. However, the pessimistic assumption can be modeled by slightly increasing $u$.
Remark that several paths with length not larger than $u^w$ may exists for a given design solution $x,y$. Then, the values of the  flow variables $f_a^w$ will describe one of them and the path choice has no influence on the objective function value \eqref{eq:MCobj}. 
Finally, constraints (\ref{eq:nat}) and (\ref{eq:nat-f}) state that variables are binary.

The \textit{Partial Covering Network Design Problem} $(PC)$, which minimizes the total construction cost of the network subject to a minimum coverage level of the total demand, can be formulated as follows:
\begin{align}
(PC) \quad \min_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z},\boldsymbol{f}} &\quad \sum_{i \in N} b_i y_i + \sum_{e \in E} c_e x_e &\label{eq:PCobj}\\ 
\mbox{s.t. }& \quad \sum_{w \in W} g^w z^w \ge \beta \, G, \label{eq:PCconst} \\
 & \quad \mbox{Constraints (\ref{rel_xy}), (\ref{flow_cons}), (\ref{Capacity}), (\ref{Utility}), (\ref{eq:nat}), (\ref{eq:nat-f}), }& \nonumber
\end{align}
\noindent where $\beta\in (0,1]$ and $G=\sum\limits_{w\in W}g^w$. Here, the objective function (\ref{eq:PCobj}) to be minimized represents the design cost. Constraint (\ref{eq:PCconst}) imposes that a proportion $\beta$ of the total demand is covered. 


In the previous works by \cite{marin2009urban} and \cite{garcia2013grasp}, constraints \eqref{Capacity} and \eqref{Utility} are formulated in a different way. For example, in \cite{garcia2013grasp}, these constraints were written as 
\begin{align}
 & f_a^w + z^w - 1 \le x_a,& \kern-2cm w \in W,\, e=\{i,j\} \in E^w: a=(i,j), \label{eq:cap_ardila} \\
 & \sum_{a\in A^w} d_a f_a^w + M(z^w -1)\le u^w z^w, & w \in W,\label{eq:uti_ardila}
\end{align}
\noindent where the design variable $x_a$ is defined for each arc. Given that $z^w-1 \le 0$, expressions \eqref{Capacity} and \eqref{Utility} are stronger than \eqref{eq:cap_ardila} and \eqref{eq:uti_ardila}, respectively. 

In addition, constraint \eqref{eq:uti_ardila} involves a \textit{``big-M''} constant. Our proposed formulation does not need it, which avoids the numerical instability generated by this constant. As we will see in Section 4.2, we observed that our proposed formulation is not only stronger than the one proposed in \cite{garcia2013grasp}, but it is also computationally more efficient. In consequence, we only focus our analysis on our proposed formulation.

Another observation is that constraints \eqref{Capacity} are a reinforcement of the usual capacity constraints $f_a^w \leq x_e$ and $f_{\hat{a}}^w \leq x_e$. In most applications where flow or design variables appear in the objective functions, the disaggregated version is sufficient to obtain a valid model as subtours are naturally non-optimal. However, it is not the case in our model, and there exist optimal solutions with subtours if the disaggregated version of \eqref{Capacity} is used. Such a strengthening was already introduced in the context of uncapacitated network design, see e.g. \cite{balakrishnan1989dual}, and Steiner trees, see e.g. \cite{sinnl2016node} and \cite{fortz2020steiner}.

\subsection{Pre-processing methods}\label{s:pre}

In this section we describe some methods to reduce the size of the instances before solving them. First, we describe how to build each subgraph $\mathcal{N}^w=(N^w,E^w)$. Then for each problem, $(MC)$ and $(PC)$, we sketch a method to eliminate O/D pairs which will never be covered.

To create $\mathcal N^w$ we only consider useful nodes and edges from $\mathcal N$. For each O/D pair $w$, we eliminate all the nodes $i\in N$ that do not belong to any path from $w^s$ to $w^t$ shorter than $u^w$. Then, we define $E^w$ as the set of edges in $E$ incident only to the non eliminated nodes. Finally, the set $A^w$ is obtained by duplicating all edges in $E^w$ with the exception of arcs $(i, w^s)$ and $(w^t,i)$. We describe this procedure in Algorithm \ref{pre_1}. 

We assume that the cost of constructing each node and each edge is not higher than the budget.

\begin{algorithm}[htpb] 
	\caption{Pre-processing I}
	\label{pre_1} 
	\begin{algorithmic} 
		\FOR{$w \in W$}
		\STATE $N^w = N$
		\FOR{$i \in N$}
		\STATE compute the shortest path for the O/D pairs $(w^s,i)$ and $(i,w^t)$
		\IF{the sum of the length of both paths is greater than $u^w$ }
		\STATE $N^w = N^w \setminus \{i \}$
		\STATE $E^w = E^w \setminus \delta(i)$
		\ENDIF
		\ENDFOR
		\STATE $A^w = \{(i,j) \in A :\{i, j\} \in E^w, \, j \neq w^s,\, i\neq w^t\}$
		\ENDFOR
 \RETURN $\{ \mathcal{N}^w = (N^w, E^w), A^w \}_{w\in W}$
\end{algorithmic}
\end{algorithm}

Next, we focus on $(MC)$. We can eliminate O/D pairs $w$ that are too expensive to be covered. That means, the O/D pair $w$ is deleted from $W$ if there is no path between $w^s$ and $w^t$ satisfying: i. its building cost is less than $C_{max}$; and ii. its length is less than $u^w$.\\
This can be checked by solving a shortest path problem with resource constraints and can thus be done in a pseudo-polynomial time. \cite{Desrochers1986algorithm} shows how to adapt Bellman-Ford algorithm to solve it. However, given the moderate size of graphs we consider, we solve it as a feasibility problem. For each $w$, we consider the feasibility problem associated to constraints (\ref{eq:budget}) (\ref{rel_xy}), (\ref{flow_cons}), (\ref{Capacity}), (\ref{Utility}) and (\ref{eq:nat}), with $z^w$ fixed to $1$. If this problem is infeasible, then the O/D pair $w$ is deleted from $W$. Otherwise, there exists a feasible path denoted by Path$_w$. We denote by $(\widetilde{N}^w, \widetilde{E}^w)$ the subgraph of $\mathcal{N}^w$ induced by Path$_w$.

\subsection{Polyhedral properties}

Both formulations $(MC)$ and $(PC)$ involve flow variables $f^w_a$ whose number can be huge when the number of O/D pairs is large. To circumvent this drawback we use a Benders decomposition approach for solving $(MC)$ and $(PC)$. In this subsection, we present properties of the two formulations that allow us to apply such a decomposition in an efficient way.
The first proposition shows that we can relax the integrality constraints on the flow variables $f^w_a$. Let $(MC\_R)$ and $(PC\_R)$ denote the formulations $(MC)$ and $(PC)$ in which constraints (\ref{eq:nat-f}) are replaced by non-negativity constraints, i.e.
\begin{equation}
f^w_a \geq 0, w \in W, a \in A. \label{eq:nneg-f}
\end{equation}
We denote the set of feasible points to a formulation $F$ by $\mathcal{F}(F)$. Further, let $Q$ be a set of points $(\boldsymbol{x},\boldsymbol{z}) \in R^q \times R^p$. 
Then the projection of $Q$ onto the 
$x$-space, denoted $Proj_xQ$, is the set of points given by $Proj_{\boldsymbol{x}} Q = \{\boldsymbol{x} \in R^q: (\boldsymbol{x},\boldsymbol{z}) \in Q$ for some $\boldsymbol{z} \in R^p\}$.

\begin{prop} \label{prop_f}
$Proj_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}(\mathcal{F}(MC)) = Proj_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}(\mathcal{F}(MC\_R))$ and $Proj_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}(\mathcal{F}(PC)) = Proj_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}(\mathcal{F}(PC\_R))$.
\end{prop}

\begin{proof} 

We provide the proof for $(MC)$, the other one being identical. 

First, $\mathcal{F}(MC) \subseteq \mathcal{F}(MC\_R)$ implies $Proj_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}(\mathcal{F}(MC)) \subseteq Proj_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}(\mathcal{F}(MC\_R))$. Second, let $(\boldsymbol{x},\boldsymbol{y},\boldsymbol{z})$ be a point belonging to $Proj_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}(\mathcal{F}(MC\_R))$. For every O/D pair $w \in W$ such that $z^w = 0$ then $\boldsymbol{f}^w=0$. In the case where $z^w=1$, there exists a flow $f^w_a \geq 0$ satisfying (\ref{flow_cons}) and (\ref{Capacity}) that can be decomposed into a convex combination of flows on paths from $w^s$ to $w^t$ and cycles. Given that the flow $f_a^w$ also satisfies (\ref{Utility}), then a flow of value 1 on one of the paths in the convex combination must satisfy this constraint. Hence by taking $f_a^w$ equal to 1 for the arcs belonging to this path and to 0 otherwise, we show that $(\boldsymbol{x},\boldsymbol{y},\boldsymbol{z})$ also belongs to $Proj_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}(\mathcal{F}(MC))$. 
\end{proof}

Note that a similar result is presented in the recent article \cite{ljubic2020benders}. Based on Proposition \ref{prop_f}, we propose a \textit{Benders decomposition} where variables $f^w_a$ are projected out from the model and replaced by {\it Benders feasibility cuts}. As we will see in Section \ref{s:facertdef}, we also consider the \textit{Benders facet-defining cuts} proposed in \cite{Conforti2019facet}. To apply this technique it is necessary to get an interior point of the convex hull of $Proj_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}(\mathcal{F}(MC\_R))$ (resp. $Proj_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}(\mathcal{F}(PC\_R))$). The following property gives us an algorithmic tool to apply this technique to $(MC)$. 


\begin{prop} \label{prop_MC}
After pre-processing, the convex hull of $Proj_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}(\mathcal{F}(MC\_R))$ is full-dimensional. 
\end{prop}

\begin{proof}
 To prove the result, we exhibit $\vert N\vert + \vert E\vert + \vert W\vert + 1$ affinely independent feasible points:
	\begin{itemize}
		\item The $0$ vector is feasible.
		\item For each $i\in N$, the points:
		$$ y_{i}=1, \, y_{i'} = 0, \, i' \in N\setminus\{i\},\quad x_e = 0,\, e\in E,\quad z^w =0, \, w\in W.$$
		\item For each $e=\{i,j\}\in E$, the points:
		$$y_k=1, \, k\in e,\, y_k = 0,\, k \in N \setminus \{i,j\},\quad x_e=1,\, x_{e'} = 0,\, e'\in E\setminus\{e\},\quad z^w =0, \, w\in W.$$
		\item For each $w\in W$, the points:
		\begin{gather*}
		y_i=1,\, i \in \widetilde{N}^w,\, y_i=0,\, i \in N\setminus \widetilde{N}^w, \quad	x_e=1, \, e\in \widetilde{E}^w,\, x_e = 0,\, e\in E\setminus\widetilde{E}^w,\\
		z^w=1,\, z^{w'} = 0, \, w'\in W\setminus\{w\}.
		\end{gather*}
	\end{itemize}
	Clearly these points are feasible and affinely independent. Thus the polytope is full-dimensional.
\end{proof}

The proof of Proposition \ref{prop_MC} gives us a way to compute an interior point of the convex hull of $Proj_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}(\mathcal{F}(MC\_R))$. The average of these $|N| + |E| + |W| + 1$ points is indeed such an interior point.

This is not the case for $(PC)$ as we show in Example $1$.

\paragraph{Example 1} Consider the instance of $(PC)$ given by the data presented in Table \ref{t:CP} and Figure \ref{fig:exPC}. We consider the case where at least half of the population must be covered, that is $\beta = 0.5$. In order to satisfy the trip coverage constraint \eqref{eq:PCconst}, the O/D pair $w=(1,4)$ must be covered. Hence $z^{(1,4)} = 1$ is an implicit equality. Furthermore, the only path with a length less than or equal to $u^{(1,4)} = 15$ is composed of edges \{1,2\} and \{2,4\}. Hence, $x_{\{1,2\}}$, $x_{\{2,4\}}$, $y_1$, $y_2$ and $y_4$ must take value $1$. In consequence, the polytope associated to $(PC)$ is not full-dimensional.

\begin{minipage}{0.45\textwidth}
\begin{table}[H]
\centering
\begin{tabular}{cccc}
\hline
 Origin & Destination & $u^w$ & $g^w$ \\
\hline
1 & 4 & 15 & 200 \\
2 & 4 & 10 & 50 \\
3 & 4 & 15 & 50 \\
\hline
\end{tabular}
\caption{Data in Example 1. We consider $\beta = 0.5$.}
\label{t:CP}
\end{table}
\end{minipage}
\begin{minipage}{0.45\textwidth}
\begin{figure}[H]
\centering
\includegraphics[width = 0.8\textwidth]{figs/examplePC}
\caption{Graph of Example 1.}
\label{fig:exPC}
\end{figure}
\end{minipage}
\\

We can compute the dimension of the convex hull of $Proj_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}(\mathcal{F}(PC\_R))$ in an algorithmic fashion. 

We find feasible affinely independent points and, at the same time, we detect O/D pairs which must be covered in any feasible solution. Due to the latter, there are a subset of nodes and a subset of edges that have to be built in any feasible solution. This means that there is a subset of design variables $y_i, i\in N$, $x_e, e\in E$ and mode choice variables $z^w, w\in W$ that must take value $1$. At the opposite to $(MC)$, a solution to $(PC)$ with all variables set to $0$ is not feasible. However, the solution obtained by serving all O/D pairs and building all nodes and edges is feasible. Therefore, we start with a solution with all variables in $\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}$ set to $1$ and we check, one by one, if it is feasible to set them to $0$. By setting one variable $x_e$ or $y_i$ to $0$, it may become impossible to cover some O/D pair $w$. In this case, we say that edge $e$ and node $i$ is \textit{essential} for $w$. To simplify the notation, we introduce the binary parameters $\theta^w_{e}$ and $\theta^w_{i}$ taking value $1$ if edge $e$ (respectively node $i$) is essential for $w$. These new points are stored in a set $L$. Each time the algorithm finds a variable that cannot be set to $0$, we store it in sets $\bar N,\, \bar E,\, \bar W$, respectively. At the end of the algorithm, the dimension of the convex hull of $Proj_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}(\mathcal{F}(PC\_R))$ is 
$$
\dim(\mathcal P_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}) = \vert N\vert + \vert E\vert + \vert W\vert - (\vert \bar{N} \vert + \vert \bar E \vert + \vert \bar{W} \vert).
$$

\noindent This procedure is depicted in Algorithm \ref{pre_2}.

\begin{algorithm}[htpb] 
	\caption{Computing the dimension of the polytope of $(PC)$} 
	\label{pre_2}
	\begin{algorithmic} 
		\STATE {\bf Initialization:} Set $\bar N = \emptyset$, $\bar E = \emptyset$, $\bar W = \emptyset$ and $L = \emptyset$ 
		\STATE Add to set $L$: $\left( y_i = 1, i\in N,\quad x_e = 1, e \in E,\quad z^w = 1, w \in W\right).$
		\FOR{$w' \in W$}
		\IF{$\sum\limits_{w \in W\setminus\{w'\}} g^w \ge \beta\, G$}
		\STATE		
		\STATE Add to set $L$:
		$\left(y_i = 1, i\in N,\quad x_e = 1, e \in E,\quad z^{w'} = 0, \, z^w = 1, w \in W\setminus\{w'\}\right).$
		\ELSE 
		\STATE $\bar W = \bar W \cup \{w'\}$ 
		\FOR{$e=\{i,j\} \in E$}
		\STATE Compute shortest path between $w'^{s}$ and $w'^{t}$ in the graph $(N^{w'}, E^{w'}\setminus\{e\})$.
		\IF{the length of the shortest path is greater than $u^{w'}$ \OR there is no path between $w'^s$ and $w'^t$}
		\STATE $\bar E = \bar E \cup \{e\}$ and $\bar N = \bar N \cup \{i,j\} $
		\ENDIF
		\ENDFOR
		\ENDIF
		\ENDFOR
		\FOR{$e' \in E\setminus \bar{E}$}
		\STATE Add to set $L$:
		$\left(y_i = 1, \, i\in N,\quad x_e = 1, e \in E\setminus \{e'\}, x_{e'}=0,\quad z^w = 1-\theta^w_{e'}, w \in W\right).$
		\ENDFOR
		\FOR{$i' \in N\setminus \bar{N}$}
		\STATE Add to set $L$:
		
		$\bigl(y_{i'}=0, \, y_i = 1, i\in N \setminus \{i'\},\quad x_e = 0, i'\in e, \, x_e = 1, i'\notin e,\quad z^w = 1-\theta^w_{i'}, w\in W\bigr).$
		\ENDFOR
		\STATE $\dim(\mathcal P_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}) = \vert N\vert + \vert E\vert + \vert W\vert - (\vert \bar N \vert + \vert \bar{E} \vert + \vert \bar W\vert).$
		\RETURN $\bar N, \,\bar E,\, \bar W$, $L$ and $\dim(conv(P_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}))$.
	\end{algorithmic}
\end{algorithm}


Algorithm \ref{pre_2} allows : i) to set some binary variables equal to $1$, decreasing the problem size; and ii) to compute a relative interior point of the convex hull of $Proj_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}(\mathcal{F}(PC\_R))$, necessary for the \textit{facet-defining cuts}, as explained below in Section \ref{s:facertdef}. The relative interior point is given by the average of the points in set $L$.

\paragraph{Example 1 cont}
Regarding the previous example and following Algorithm \ref{pre_2}, the O/D pair $(1,4)$ must be covered, $z^{(1,4)}=1$. Due to that, as its shortest path in the networks $(N^{(1,4)}, E^{(1,4)}\setminus\{\{1,2\}\})$ and $(N^{(1,4)}, E^{(1,4)}\setminus\{\{2,4\}\})$ is greater than $u^{(1,4)}=15$, variables $x_{\{1,2\}}$, $x_{\{2,4\}}$, $y_1$, $y_2$, $y_4$ are set to $1$. Finally, the dimension of this polyhedron is
$$\dim(P_{\boldsymbol{x},\boldsymbol{y},\boldsymbol{z}}) = 4+4+3-(3+2+1)=5.$$

The relative interior point computed is:
\begin{align*}
\,x_{\{1,2\}} = 1,\,\,x_{\{2,4\}} = 1, x_{\{1,3\}} = \frac{5}{6}, \,x_{\{3,4\}} = \frac{2}{3},\, y_1 = 1,\, y_2 = 1,\, y_3 = \frac{5}{6},\, y_4 = \frac{5}{6},\\
z^{(1,4)} = 1,\,z^{(2,4)} = \frac{5}{6},\,z^{(3,4)} = \frac{1}{2}.
\end{align*}

\subsection{Setting an initial solution} \label{s:initial_solution}


We determine an initial feasible solution for $(MC)$ and $(PC)$ with a simple greedy heuristic in which we sequentially select O/D pairs with best ratio demand overbuilding cost. More precisely, given the potential network $\mathcal{N} = (N,E)$, we compute for each O/D pair $w$ the ratio $r_w = \frac{g^w}{C(\mbox{Path}_w)}$, where $C(\mbox{Path}_w)$ is the cost of a feasible path for $w$. We order these ratios decreasingly. We use this initial order in the heuristic for both $(MC)$ and $(PC)$.
For $(MC)$ the method proceeds as follows. It starts with an empty list of built nodes and edges, an empty list of O/D pairs covered, and a total cost set to $0$. For each O/D pair $w$, in decreasing order of $r_w$, the heuristic tries to build Path$_w$ considering edges and nodes that are already built. If the additional cost plus the current cost is less than the budget $C_{max}$, nodes and edges in Path$_w$ are built and the O/D pair $w$ is covered (i.e. $z^w = 1$). The total cost, the lists of built nodes and edges are updated. Otherwise we proceed with the next O/D pair. At the end of the algorithm we have an initial feasible solution.

To get an initial solution for $(PC)$ we start with a list of all the O/D pairs covered and the amount of population covered equal to $G$. For each O/D pair $w$, in decreasing order of $r_w$, the algorithm checks if by deleting the O/D pair $w$ from the list, the coverage constraint (\ref{eq:PCconst}) is satisfied. If so, the O/D pair $w$ is deleted from the list and the amount of population covered is updated. Finally, the algorithm builds the union of the subgraphs $(\widetilde{N}^w,\widetilde{E}^w)$ induced by Path$_w$ for all the O/D pairs covered. Note that both initial solutions can be computed by solving $\vert W \vert$ shortest paths problems. These tasks can be executed  much faster  than solving  $(MC)$ and $(PC)$ to optimality.

Pseudo-codes for both routines are provided in \ref{ap:mipstart}. In Section \ref{s:computational}, we will show the efficiency of adding this initial solution at the beginning of the branch-and-Benders-cut procedure.


==> paper Benders Decomposition draft ArXiv - tercera versi�n/old_tables.tex <==
\begin{table}[htpb]
\centering
\begin{tabular}{cccccc}
\cline{2-6}
 & \texttt{CPLEX}& \texttt{Auto\_BD} & \texttt{BD\_Trd} & \texttt{BD\_Norm} & \texttt{BD\_CW}\\ \hline
 without \texttt{CS} &3& 10 & 9 & 8 & 8 \\ 
\texttt{+CS}& - & 10 & 10 & 10 & 10 \\ \hline
\end{tabular}\caption{Instances N40 solved for $(MC)$ within a time limit of 1 hour.}
\label{table:optMC}
\end{table}

\begin{table}[htpb]
\centering
\begin{tabular}{cccccc}
\cline{2-6}
 & \texttt{CPLEX}& \texttt{Auto\_BD} & \texttt{BD\_Trd} & \texttt{BD\_Norm} & \texttt{BD\_CW}\\ \hline
 without \texttt{CS}&3& 9 & 8 & 8 & 8 \\ %\hline
\texttt{+CS} & - & 10 & 10 & 10 & 10 \\ \hline
\end{tabular}\caption{Instances N40 solved for $(PC)$ within a time limit of 1 hour.}
\label{table:optPC}
\end{table}

\begin{table}[htpb]
\centering
\begin{tabular}{c c c cc cc cc cc}
\cline{2-11}% \hline
&\multirow{2}{*}{Network} & \texttt{CPLEX} & \multicolumn{2}{c}{\texttt{Auto\_BD}} & \multicolumn{2}{c}{\texttt{BD\_Trd}} & \multicolumn{2}{c}{\texttt{BD\_Norm}} & \multicolumn{2}{c}{\texttt{BD\_CW}} \\ \cline{3-11} 
 & & \texttt{t} & \texttt{t} & \texttt{cuts} & \texttt{t} & \texttt{cuts} & \texttt{t} & \texttt{cuts} & \texttt{t} & \texttt{cuts} \\ \hline
\multirow{3}{1cm}{\centering{without \texttt{CS}}} & N10 & 0.18 & 0.43 & 27 & 0.25 & 92 & 0.24 & 91 & 0.19 & 94 \\ 
& N20 & 6.77 & 4.51 & 273 & 3.89 & 620 & 3.18 & 590 & 3.34 & 641 \\ 
& N40 & 1646.93 & 617.85 & 1967 & 1095.25 & 3990 & 541.03 & 3677 & 457.81 & 4137 \\ \hline
\multirow{3}{*}{\texttt{+CS}}& N10 & - & 0.32 & 12 & 0.21 & 49 & 0.28 & 52 & 0.23 & 54 \\ 
& N20 & - & 3.94 & 178 & 2.29 & 382 & 2.50 & 383 & 1.85 & 416 \\
& N40 & - & 484.95 & 1248 & 637.49 & 2378 & 575.87 & 2530 & 272.39 & 3186 \\ \hline
\end{tabular}\caption{Comparing the performance of the three algorithms for $(MC)$.}
\label{table: MC 1}
\end{table}

\begin{table}[htpb]
\centering
\begin{tabular}{c c c cc cc cc cc}
\cline{2-11}
& \multirow{2}{*}{Network} & \texttt{CPLEX} & \multicolumn{2}{c}{\texttt{Auto\_BD}} & \multicolumn{2}{c}{\texttt{BD\_Trd}} & \multicolumn{2}{c}{\texttt{BD\_Norm}} & \multicolumn{2}{c}{\texttt{BD\_CW}} \\ \cline{3-11} 
 & & \texttt{t}& \texttt{t} & \texttt{cuts} & \texttt{t} & \texttt{cuts} & \texttt{t} & \texttt{cuts} & \texttt{t} & \texttt{cuts} \\ \hline
 \multirow{3}{1.3cm}{\centering{without \texttt{CS}}} & N10 & 0.18 & 0.29 & 16 & 0.24 & 92 & 0.28 & 89 & 0.20 & 91 \\ %\hline
 & N20 & 6.73 & 4.87 & 305 & 3.55 & 607 & 4.68 & 681 & 2.15 & 606 \\ %\hline
& N40 & 2153.15 & 504.06 & 1752 & 657.59 & 4470 & 514.42 & 4246 & 837.41 & 4412 \\ \hline
\multirow{3}{*}{\texttt{+CS}}& N10 & - & 0.28 & 11 & 0.16 & 56 & 0.20 & 57 & 0.145 & 54 \\
& N20& - & 4.12 & 213 & 3.11 & 497 & 3.43 & 495 & 2.070 & 461 \\
& N40 & - & 439.23 & 1527 & 261.74 & 3528 & 323.21 & 3583 & 197.55 & 3949 \\ \hline
\end{tabular}
\caption{Comparing the performance of the three algorithms for $(PC)$.}
\label{table: PC 1}
\end{table}














\begin{table}[htpb]
\centering
\begin{tabular}{c cc cc cc cc}
\cline{2-9}
& \multicolumn{2}{c}{\texttt{Auto\_BD}} & \multicolumn{2}{c}{\texttt{BD\_Trd}} & \multicolumn{2}{c}{\texttt{BD\_Norm}} & \multicolumn{2}{c}{\texttt{BD\_CW}} \\ \cline{2-9} 
& \texttt{gap} & \texttt{cuts} & \texttt{gap} & \texttt{cuts} & \texttt{gap} & \texttt{cuts} & \texttt{gap} & \texttt{cuts} \\ \hline
without\{\texttt{CS}, \texttt{IS}, \texttt{RNC}\}& 38.54 & 6545 & 45.68 & 14068 & 44.53 & 13340 & 43.77 & 16707 \\ 
\texttt{+CS}& 30.06 & 3729 & 24.27 & 8754 & 22.17 & 8912 & 25.76 & 11378 \\ 
\texttt{+CS+IS} & 32.90 & 4987 & 27.23 & 9038 & 26.94 & 9469 & 22.27 & 11151 \\
\texttt{+CS+IS+RNC} &\multicolumn{2}{c}{-}& 37.88 & 8054 & 37.92 & 8230 & 33.58 & 10834 \\ \hline
\end{tabular}\caption{Computing gaps to solve N60 $(MC)$ instances comparing the performance of three families of Benders cuts.}
\label{table:MC 2}
\end{table}



\begin{table}[htpb]
\centering
\begin{tabular}{c cc cc cc cc}
\cline{2-9}
& \multicolumn{2}{c}{\texttt{Auto\_BD}} & \multicolumn{2}{c}{\texttt{BD\_Trd}} & \multicolumn{2}{c}{\texttt{BD\_Norm}} & \multicolumn{2}{c}{\texttt{BD\_CW}} \\ \cline{2-9} 
& \texttt{gap} & \texttt{cuts} & \texttt{gap} & \texttt{cuts} & \texttt{gap} & \texttt{cuts} & \texttt{gap} & \texttt{cuts} \\ \hline
without\{\texttt{CS}, \texttt{IS}, \texttt{RNC}\} & 20.49 & 7009 & 20.40 & 14784 & 21.41 & 15501 & 19.93 & 15116 \\ %\cline{1-3}
\texttt{+CS} & 15.92 & 5109 & 14.89 & 12354 & 14.09 & 11687 & 14.50 & 11744 \\ %\cline{2-3}
\texttt{+CS+IS} & 15.86 & 4372& 11.06 & 8961 & 10.47 & 8490 & 10.44 & 9683 \\ %\cline{3-3}
\texttt{+CS+IS+RNC} &\multicolumn{2}{c}{-} & 20.93 & 10971 & 21.28 & 11449 & 19.94 & 11053 \\ \hline
\end{tabular}\caption{Computing gaps to solve N60 $(PC)$ instances comparing the performance of three families of Benders cuts.}
\label{table:PC 2}
\end{table}

==> paper Benders Decomposition draft ArXiv - tercera versi�n/tablasN102040.tex <==
\begin{table}[htpb]
\footnotesize
\centering
\begin{tabular}{c c c c cc cc cc cc}
\cline{2-12}% \hline
&&\multirow{2}{*}{Network} & \texttt{CPLEX} &\multicolumn{2}{c}{\texttt{Auto\_BD}} & \multicolumn{2}{c}{\texttt{BD\_Trd}} & \multicolumn{2}{c}{\texttt{BD\_Norm}} & \multicolumn{2}{c}{\texttt{BD\_CW}} \\
\cline{4-12} 
&& & \texttt{t} & \texttt{t} & \texttt{cuts} & \texttt{t} & \texttt{cuts} & \texttt{t} & \texttt{cuts} & \texttt{t} & \texttt{cuts} \\ \hline
\multirow{6}{*}{$(MC)$} &\multirow{3}{0.5cm}{\centering{w.o. \texttt{CS}}} & N10 & 0.18 & 0.43 & 27 & 0.25 & 92 & 0.24 & 91 & 0.19 & 94 \\ 
&& N20 & 6.77 & 4.51 & 273 & 3.89 & 620 & 3.18 & 590 & 3.34 & 641 \\ 
&& N40 & 1646.93 & 617.85 & 1967 & 1095.25 & 3990 & 541.03 & 3677 & 457.81 & 4137 \\ \cline{2-12} 
&\multirow{3}{*}{\texttt{+CS}}& N10 & - & 0.32 & 12 & 0.21 & 49 & 0.28 & 52 & 0.23 & 54 \\ 
&& N20 & - & 3.94 & 178 & 2.29 & 382 & 2.50 & 383 & 1.85 & 416 \\
&& N40 & - & 484.95 & 1248 & 637.49 & 2378 & 575.87 & 2530 & 272.39 & 3186 \\ \hline
\multirow{6}{*}{$(PC)$} &\multirow{3}{0.5cm}{\centering{w.o. \texttt{CS}}} & N10 & 0.18 & 0.29 & 16 & 0.24 & 92 & 0.28 & 89 & 0.20 & 91 \\ %\hline
 && N20 & 6.73 & 4.87 & 305 & 3.55 & 607 & 4.68 & 681 & 2.15 & 606 \\ %\hline
&& N40 & 2153.15 & 504.06 & 1752 & 657.59 & 4470 & 514.42 & 4246 & 837.41 & 4412 \\  \cline{2-12} 
&\multirow{3}{*}{\texttt{+CS}}& N10 & - & 0.28 & 11 & 0.16 & 56 & 0.20 & 57 & 0.145 & 54 \\
&& N20& - & 4.12 & 213 & 3.11 & 497 & 3.43 & 495 & 2.070 & 461 \\
&& N40 & - & 439.23 & 1527 & 261.74 & 3528 & 323.21 & 3583 & 197.55 & 3949 \\ \hline
\end{tabular}
\caption{Comparing the performance of the three algorithms for $(MC)$ and $(PC)$.}
\label{table:perfN102040}
\end{table}


==> paper Benders Decomposition draft ArXiv - tercera versi�n/tablasN60.tex <==
\begin{table}[htpb]
\small
\centering
\begin{tabular}{c c cc cc cc cc}
\cline{3-10}
&& \multicolumn{2}{c}{\texttt{Auto\_BD}} & \multicolumn{2}{c}{\texttt{BD\_Trd}} & \multicolumn{2}{c}{\texttt{BD\_Norm}} & \multicolumn{2}{c}{\texttt{BD\_CW}} \\ \cline{3-10} 
&& \texttt{gap} & \texttt{cuts} & \texttt{gap} & \texttt{cuts} & \texttt{gap} & \texttt{cuts} & \texttt{gap} & \texttt{cuts} \\ \hline
\multirow{4}{*}{$(MC)$}&without\{\texttt{CS}, \texttt{IS}, \texttt{RNC}\}& 38.54 & 6545 & 45.68 & 14068 & 44.53 & 13340 & 43.77 & 16707 \\ 
&\texttt{+CS}& 30.06 & 3729 & 24.27 & 8754 & 22.17 & 8912 & 25.76 & 11378 \\ 
&\texttt{+CS+IS} & 32.90 & 4987 & 27.23 & 9038 & 26.94 & 9469 & 22.27 & 11151 \\
&\texttt{+CS+IS+RNC} &\multicolumn{2}{c}{-}& 37.88 & 8054 & 37.92 & 8230 & 33.58 & 10834 \\ \hline
\multirow{4}{*}{$(PC)$}&without\{\texttt{CS}, \texttt{IS}, \texttt{RNC}\} & 20.49 & 7009 & 20.40 & 14784 & 21.41 & 15501 & 19.93 & 15116 \\ %\cline{1-3}
&\texttt{+CS} & 15.92 & 5109 & 14.89 & 12354 & 14.09 & 11687 & 14.50 & 11744 \\ %\cline{2-3}
&\texttt{+CS+IS} & 15.86 & 4372& 11.06 & 8961 & 10.47 & 8490 & 10.44 & 9683 \\ %\cline{3-3}
&\texttt{+CS+IS+RNC} &\multicolumn{2}{c}{-} & 20.93 & 10971 & 21.28 & 11449 & 19.94 & 11053 \\ \hline
\end{tabular}\caption{Computing gaps to solve N60 for $(MC)$ and $(PC)$ instances comparing the performance of three families of Benders cuts.}
\label{table:n60}
\end{table}
